Wave propagation in micromorphic anisotropic continua with an application to tetragonal crystals

We study the coupled macroscopic and lattice wave propagation in anisotropic crystals seen as continua with affine microstructure (or micromorphic). In the general case we obtain qualitative informations on the frequencies and the dispersion realtions. These results are then specialized to crystals of the tetragonal point group for various propagation directions: exact representation for the acoustic and optic frequencies and for the coupled vibrations modes are obtained for propagation directions along the tetragonal c-axis.

==> leftovers/66M1.tex <==
\section{Autovalori in M1}

\begin{align}
A&=\nonumber\\
B&=2b^2+c^2+2 l^2+2 m^2+n^2+p^2+2 q^2-a d+a e-a f-d f+e f-a g-d g+e g-f g-a h-d h+e h-g h+2 n p\nonumber\\
C&=\left(-2 b^2-c^2-2 l^2-2 m^2-n^2-p^2-2 q^2+a d-a e+a f+d f-e f+a g+d g-e g+f g+a h+d h-e h+g h-2 n p\right)\nonumber\\
D&=\left(2 d b^2-2 e b^2+2 g b^2-4 c l b-4 n q b-4 p q b+2 a l^2+2 d l^2-2 e l^2+2 a m^2+2 f m^2+2 h m^2+a n^2+g n^2+a p^2+g p^2+2 f q^2+2 g q^2+2 h q^2+c^2 d-c^2 e+c^2 f-a d f+a e f-a d g+a e g-a f g-d f g+e f g+c^2 h-a d h+a e h-a g h-d g h+e g h-4 l m n-4 l m p+2 a n p+2 g n p-4 c m q\right)\nonumber\\
E&=\left(4 m^2 b^2-2 d g b^2+2 e g b^2+4 c d l b-4 c e l b-4 c m n b-4 c m p b-8 l m q b+4 g n q b+4 g p q b-2 a d l^2+2 a e l^2-2 a f m^2-2 a h m^2+c^2 n^2-a g n^2+c^2 p^2-a g p^2+4 l^2 q^2-2 f g q^2-2 g h q^2-c^2 d f+c^2 e f+a d f g-a e f g-c^2 d h+c^2 e h+a d g h-a e g h+4 a l m n+4 a l m p+2 c^2 n p-2 a g n p+4 c f m q+4 c h m q-4 c l n q-4 c l p q\right)\nonumber\\
P&=2 C^3-9 A D C-72 E C+27 D^2+27 A^2 E\nonumber\\
Q&=\left(C^2-3 A D+12 E\right)\nonumber\\
W&=\frac{\sqrt[3]{P+\sqrt{P^2-4 Q^3}}}{3 \sqrt[3]{2}}+\frac{\sqrt[3]{2} Q}{3 \sqrt[3]{P+\sqrt{P^2-4 Q^3}}}\nonumber\\
K_{o}&=\frac{1}{4} A^2+B+\frac{1}{3} C+W\nonumber\\
K_{1}&=\frac{1}{2} A^2+\frac{4}{3} B-W\nonumber\\
K_{2}&=\frac{-A^3+4 C A-8 D}{4 K}\nonumber
\end{align}

\begin{align}
\omega_{3}^{2}&=\frac{1}{4} A-\frac{1}{2} \sqrt{K_{o}}-\frac{1}{2} \sqrt{K_{1}-K_{2}}\nonumber\\
\omega_{4}^{2}&=\frac{1}{4} A-\frac{1}{2} \sqrt{K_{o}}+\frac{1}{2} \sqrt{K_{1}-K_{2}}\nonumber\\
\omega_{5}^{2}&=\frac{1}{4} A+\frac{1}{2} \sqrt{K_{o}}-\frac{1}{2} \sqrt{K_{1}+K_{2}}\nonumber\\
\omega_{6}^{2}&=\frac{1}{4} A+\frac{1}{2} \sqrt{K_{o}}+\frac{1}{2} \sqrt{K_{1}+K_{2}}\nonumber
\end{align}

==> leftovers/auto.tex <==
\section{Fourth-order}

\begin{align}
&\omega^{2} _1=f-h \nonumber\\
&\omega^{2} _2=\frac{1}{3} (a+f+g+h)+\frac{
\sqrt[3]{
A+\sqrt{
4B^3+A^2}}}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2}B}{3 \sqrt[3]{A+\sqrt{4B^3+A^2}}}\nonumber\\
&\omega^{2} _3=\frac{1}{3} (a+f+g+h)-\frac{\left(1-i \sqrt{3}\right) \sqrt[3]{A+\sqrt{4B^3+A^2}}}{6 \sqrt[3]{2}}+\frac{\left(1+i \sqrt{3}\right) B}{3 \times 2^{2/3} \sqrt[3]{A+\sqrt{4B^3+A^2}}} \\ 
&\omega^{2} _4=\frac{1}{3} (a+f+g+h)-\frac{\left(1+i \sqrt{3}\right) \sqrt[3]{A+\sqrt{4B^3+A^2}}}{6 \sqrt[3]{2}}+\frac{\left(1-i \sqrt{3}\right) B}{3 \times 2^{2/3} \sqrt[3]{A+\sqrt{4 B^3+A^2}}}\nonumber
\end{align}

\begin{align}
&A=2 a^3-3 f a^2-3 g a^2-3 h a^2-3 f^2 a-3 g^2 a-3 h^2 a-36 l^2 a+18 b d a+9 c e a+12 f g a-6 f h a+12 g h a+2 f^3\nonumber\\
&+2 g^3+2 h^3-3 f g^2+6 f h^2-3 g h^2+18 f l^2+18 g l^2+18 h l^2+18 b d f-18 c e f-3 f^2 g-36 b d g+9 c e g+6 f^2 h\nonumber\\
&-3 g^2 h+18 b d h-18 c e h-6 f g h+54 c d l+54 b e l\nonumber\\
&B= 3\left(-2 l^2-2 b d-c e+a f+a g+f g+a h+g h\right)-(a+f+g+h)^2\nonumber
\end{align}

\begin{align}
&w_{1}=\{0,-1,1,0\} \nonumber\\ 
&w_{2}=\Bigg\{1,-H_{1}K_{1},-H_{1}K_{1},H_{1}\Bigg\} \nonumber\\
&w_{3}=\Bigg\{1,-H_{2}\frac{E+d K_{2}}{F-e K_{2}},-H_{2}\frac{E+d K_{2}}{F-e K_{2}},H_{2}\Bigg\} \nonumber\\
&w_{4}=\Bigg\{1,-H_{3}\frac{E+d K_{3}}{F-e K_{3}},-H_{3}\frac{E+d K_{3}}{F-e K_{3}},H_{3}\Bigg\}\nonumber
\end{align}

\begin{align}
C&=a+f+g+h\nonumber\\
D&=\sqrt[3]{A+\sqrt{4B^3+A^2}}\nonumber\\
E&=-d g+e l\nonumber\\
F&=e f+e h-2 d l\nonumber
\end{align}
\begin{align}
K_{1}&=\frac{E+d \left(\frac{1}{3} C+\frac{D}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} B}{3 D}\right)}{F-e \left(\frac{1}{3} C+\frac{D}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} B}{3 D}\right)}\nonumber\\
K_{2}&=\frac{1}{3} C-\frac{\left(1-i \sqrt{3}\right) D}{6 \sqrt[3]{2}}+\frac{\left(1+i \sqrt{3}\right) B}{3 \times 2^{2/3} D}\nonumber\\
K_{3}&=\frac{1}{3} C-\frac{\left(1+i \sqrt{3}\right) D}{6 \sqrt[3]{2}}+\frac{\left(1-i \sqrt{3}\right) B}{3 \times 2^{2/3} D}\nonumber
\end{align}

\begin{align}
H_{1}^{-1}&=\frac{2l}{e}K_{1}-\frac{g-\frac{1}{3}C-\frac{D}{3 \sqrt[3]{2}}+\frac{\sqrt[3]{2} B}{3 D}}{e}\,,\nonumber\\
H_{2}^{-1}&=\frac{2 l \left(E+d K_{2}\right)}{e \left(F-e K_{2}\right)}-\frac{g-K_{2}}{e}\,,\nonumber\\
H_{3}^{-1}&=\frac{2 l \left(E+d K_{3}\right)}{e \left(F-e K_{3}\right)}-\frac{g-K_{3}}{e}\,,\nonumber
\end{align}

\begin{align}
&a f^2 g-a f^2 w-2 a f g w-2 a f l^2+2 a f w^2-a g h^2+a g w^2+a h^2 w+2 a h l^2+2 a l^2 w-a w^3-2 b^2 f g+2 b^2 f w+2 b^2 g h+2 b^2 g w\nonumber\\
&-2 b^2 h w-2 b^2 w^2+4 b c f l-4 b c h l-4 b c l w-c^2 f^2+2 c^2 f w+c^2 h^2-c^2 w^2-f^2 g w+f^2 w^2+2 f g w^2+2 f l^2 w-2 f w^3\nonumber\\
&+g h^2 w-g w^3-h^2 w^2-2 h l^2 w-2 l^2 w^2+w^4=0\nonumber
\end{align}

\begin{align}
&w^4+w^3(-a-2 f-g)+w^2(-2 l^2 +2 a f +a g +f^2 +2 f g -c^2 -2 b^2 -h^2 )\nonumber\\
&+w(-a f^2 -2 a f g +a h^2 +2 a l^2 +2 b^2 f +2 b^2 g -2 b^2 h -4 b c l -f^2 g +2 f l^2 +2 c^2 f -2 h l^2 +g h^2 )\nonumber\\
&+a f^2 g-2 a f l^2-a g h^2+2 a h l^2-2 b^2 f g+2 b^2 g h+4 b c f l-4 b c h l-c^2 f^2+c^2 h^2=0\nonumber
\end{align}
\begin{equation}
(w-f+h)(Aw^{3}+Bw^{2}+Cw+D)=0
\end{equation}
\begin{equation}
(Aw^{4}+(B+(h-f)A)w^{3}+(C+(h-f)B)w^{2}+(D+(h-f)C)w+(h-f)D)=0
\end{equation}

Qui a, b, c, d devono essere maiuscoli.

\begin{align}
&x=\frac{\sqrt[3]{\sqrt{\left(-27 a^2 d+9 a b c-2 b^3\right)^2+4 \left(3 a c-b^2\right)^3}-27 a^2 d+9 a b c-2 b^3}}{3 \sqrt[3]{2} a}\nonumber\\
&-\frac{\sqrt[3]{2} \left(3 a c-b^2\right)}{3 a \sqrt[3]{\sqrt{\left(-27 a^2 d+9 a b c-2 b^3\right)^2+4 \left(3 a c-b^2\right)^3}-27 a^2 d+9 a b c-2 b^3}}-\frac{b}{3 a}\nonumber\\
&{\rm {OR}}\nonumber\\
&x=-\frac{\left(1-i \sqrt{3}\right) \sqrt[3]{\sqrt{\left(-27 a^2 d+9 a b c-2 b^3\right)^2+4 \left(3 a c-b^2\right)^3}-27 a^2 d+9 a b c-2 b^3}}{6 \sqrt[3]{2} a}\nonumber\\
&+\frac{\left(1+i \sqrt{3}\right) \left(3 a c-b^2\right)}{3 \times 2^{2/3} a \sqrt[3]{\sqrt{\left(-27 a^2 d+9 a b c-2 b^3\right)^2+4 \left(3 a c-b^2\right)^3}-27 a^2 d+9 a b c-2 b^3}}-\frac{b}{3 a}\nonumber\\
&{\rm {OR}}\nonumber\\
&x=-\frac{\left(1+i \sqrt{3}\right) \sqrt[3]{\sqrt{\left(-27 a^2 d+9 a b c-2 b^3\right)^2+4 \left(3 a c-b^2\right)^3}-27 a^2 d+9 a b c-2 b^3}}{6 \sqrt[3]{2} a}\nonumber\\
&+\frac{\left(1-i \sqrt{3}\right) \left(3 a c-b^2\right)}{3 \times 2^{2/3} a \sqrt[3]{\sqrt{\left(-27 a^2 d+9 a b c-2 b^3\right)^2+4 \left(3 a c-b^2\right)^3}-27 a^2 d+9 a b c-2 b^3}}-\frac{b}{3 a}\nonumber
\end{align}


\begin{align} 
&\lambda _1\to 0 \\ 
&\lambda _2\to f-h \\ 
&\lambda _3\to \frac{1}{2} \left(-\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}+f+g+h\right) \\ 
&\lambda _4\to \frac{1}{2} \left(\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}+f+g+h\right) \\ 
&{v_1}= \{1,0,0,0\} \\ 
&{v_2}= \{0,-1,1,0\} \\ 
&{v_3}=\{0,\frac{l^2-h \left(\frac{1}{2} \left(\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}-f-g-h\right)+g\right)}{\frac{1}{2} l \sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}+\frac{f l}{2}-\frac{g l}{2}-\frac{3 h l}{2}}-\frac{\frac{1}{2} \left(\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}-f-g-h\right)+g}{l},\\
&-\frac{l^2-h \left(\frac{1}{2} \left(\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}-f-g-h\right)+g\right)}{\frac{1}{2} l \sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}+\frac{f l}{2}-\frac{g l}{2}-\frac{3 h l}{2}},1\} \\ 
&{v_4}=\{0,\frac{l^2-h \left(\frac{1}{2} \left(-\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}-f-g-h\right)+g\right)}{-\frac{1}{2} l \sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}+\frac{f l}{2}-\frac{g l}{2}-\frac{3 h l}{2}}-\frac{\frac{1}{2} \left(-\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}-f-g-h\right)+g}{l},\\
&-\frac{l^2-h \left(\frac{1}{2} \left(-\sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}-f-g-h\right)+g\right)}{-\frac{1}{2} l \sqrt{f^2-2 f g+2 f h+g^2-2 g h+h^2+8 l^2}+\frac{f l}{2}-\frac{g l}{2}-\frac{3 h l}{2}},1\} 
\end{align}

\section{Fifth-order}
\begin{align}
A&=a+c-d+f\,,\nonumber\\
B&=-a+c+d+f\,,\nonumber\\
C&=g-h\,,\nonumber\\
D&=a+b+c+d-f\,,\nonumber
\end{align}
\begin{align}
E&=2 b^3+2 c^3+2 d^3-2 f^3-3 b c^2-3 b d^2-3 c d^2+18 b e^2-36 c e^2+18 d e^2-3 b f^2\nonumber\\
&+6 c f^2-3 d f^2-18 b g^2+9 c g^2+9 d g^2-9 f g^2-18 b h^2+9 c h^2+9 d h^2-9 f h^2\\&+18 b l^2+18 c l^2-36 d l^2-18 f l^2-3 b^2 c-3 b^2 d-3 c^2 d+12 b c d+3 b^2 f-6 c^2 f\nonumber\\
&+3 d^2 f+36 e^2 f+6 b c f-12 b d f+6 c d f-36 b g h+18 c g h+18 d g h\nonumber\\
&-18 f g h+108 e g l+108 e h l\,,\nonumber\\
F&=c^2+b^2-2d^2-9e^2+f^2-3g^2-3h^2 +18 l^2-6 b c +3 b d +3 c d\nonumber\\
&+4 b f -2 c f -2 d f -9 g h\,,\nonumber\\
G&=2 a^3-3 b a^2-3 c a^2+6 d a^2+3 f a^2-3 b^2 a-3 c^2 a+6 d^2 a+18 e^2 a-3 f^2 a\nonumber\\
&+9 g^2 a+9 h^2 a-36 l^2 a+12 b c a-6 b d a-6 c d a-12 b f a+6 c f a+6 d f a+18 g h a\,,\nonumber\\
H&=-2 e^2-g^2-h^2-2 l^2+a b+a c+b c+b d+c d-a f-b f-d f-2 g h\nonumber
\end{align}
\begin{equation}
Q=\sqrt{4 \left(3H-D^2\right)^3+\left(G+E\right)^2}
\end{equation}



\begin{align}
&\omega_{1}^{2}=\frac{1}{2} \left(A-\sqrt{B^2+4C}\right)\,,\nonumber\\
&\omega_{2}^{2}=\frac{1}{2} \left(A+\sqrt{B^2+4C}\right)\,,\nonumber\\
&\omega_{3}^{2}=\frac{1}{3} D+\frac{\sqrt[3]{G+E+Q}}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} \left(3H-D^2\right)}{3 \sqrt[3]{G+E+Q}}\,,\nonumber\\
&\omega_{4}^{2}=\frac{1}{3} D-\frac{\left(1-i \sqrt{3}\right) \sqrt[3]{G+E+Q}}{6 \sqrt[3]{2}}+\frac{\left(1+i \sqrt{3}\right) \left(3H-D^2\right)}{3 \times 2^{2/3} \sqrt[3]{G+E+Q}}\,,\nonumber\\
&\omega_{5}^{2}=\frac{1}{3} D-\frac{\left(1+i \sqrt{3}\right) \sqrt[3]{G+E+Q}}{6 \sqrt[3]{2}}+\frac{\left(1-i \sqrt{3}\right) \left(3H-D^2\right)}{3 \times 2^{2/3} \sqrt[3]{G+E+Q}}\,,\nonumber
\end{align}

\begin{align}
&-w^5\nonumber\\
&+(2 a +b+2 c)w^4\nonumber\\
&+(-a^2 -c^2 +d^2 +2 e^2 +f^2 +2 g^2 +2 h^2 +2 l^2 -2 a b -4 a c -2 b c)w^3\nonumber\\
&+(2 a c^2 +b c^2 -b d^2 -2 c d^2 -2 a e^2 -4 c e^2 +2 d e^2 -2 a f^2 -b f^2 -2 a g^2 -2 b g^2 -2 c g^2 -2 a h^2\nonumber\\
& -2 b h^2 -2 c h^2 -4 a l^2 -2 c l^2 -2 f l^2 +a^2 b +2 a^2 c +4 a b c +4 d g h -4 f g h +4 e g l +4 e h l )w^2\nonumber\\
&+(-g^4 -h^4 -a^2 c^2 -2 a b c^2 +c^2 d^2 +2 b c d^2 +2 c^2 e^2 +4 a c e^2 -4 c d e^2 +a^2 f^2 -d^2 f^2 -2 e^2 f^2\nonumber\\
& +2 a b f^2 -2 e^2 g^2 +2 a b g^2 +2 a c g^2 +2 b c g^2 -2 d f g^2 -2 e^2 h^2 +2 g^2 h^2 +2 a b h^2 +2 a c h^2 \nonumber\\
&+2 b c h^2 -2 d f h^2 +2 a^2 l^2 -2 d^2 l^2 -2 g^2 l^2 -2 h^2 l^2 +4 a c l^2 +4 a f l^2 +4 g h l^2 -2 a^2 b c +4 e^2 g h\nonumber\\
& -4 b d g h -4 c d g h +4 a f g h +4 b f g h -4 a e g l -4 c e g l +4 d e g l\nonumber\\
& -4 e f g l -4 a e h l -4 c e h l +4 d e h l -4 e f h l )w\nonumber\\
&+b g^4+b h^4+a^2 b c^2-b c^2 d^2-2 a c^2 e^2+2 c^2 d e^2+b d^2 f^2+2 a e^2 f^2-2 d e^2 f^2-a^2 b f^2\nonumber\\
&+2 c e^2 g^2-2 a b c g^2-2 e^2 f g^2+2 b d f g^2+2 c e^2 h^2-2 b g^2 h^2-2 a b c h^2\nonumber\\
&-2 e^2 f h^2+2 b d f h^2+2 c d^2 l^2+2 a g^2 l^2+2 d g^2 l^2+2 a h^2 l^2\nonumber\\
&+2 d h^2 l^2-2 a^2 c l^2-2 a^2 f l^2+2 d^2 f l^2-4 a g h l^2-4 d g h l^2-4 c e^2 g h+4 b c d g h\nonumber\\
&+4 e^2 f g h-4 a b f g h-4 e g^3 l-4 e h^3 l+4 e g h^2 l+4 a c e g l-4 c d e g l+4 a e f g l\nonumber\\
&-4 d e f g l+4 e g^2 h l+4 a c e h l-4 c d e h l+4 a e f h l-4 d e f h l =0
\end{align}

\section{sixth order}

\begin{align}
A&=a+b+e+f\nonumber\\
B&=a-b+e+f\nonumber\\
C&=2 a^3+6 b a^2-3 e a^2-3 f a^2+6 b^2 a+9 c^2 a+9 d^2 a-3 e^2 a-3 f^2 a-18 g^2 a-6 b e a-6 b f a\nonumber\\
&+12 e f a+2 b^3+2 e^3+2 f^3+9 b c^2+9 b d^2-3 b e^2-3 b f^2-3 e f^2-18 b g^2+9 e g^2+9 f g^2\nonumber\\
&-3 b^2 e+9 c^2 e-18 d^2 e-3 b^2 f-18 c^2 f+9 d^2 f-3 e^2 f+12 b e f+54 c d g\nonumber\\
D&=-c^2-d^2-g^2+a e+b e+a f+b f+e f\nonumber\\
E&=-c^2-d^2-g^2+a e-b e+a f-b f+e f\nonumber
\end{align}

\begin{align}
P&=\sqrt[3]{C+\sqrt{4 \left(3 D-A^2\right)^3+C^2}}\nonumber\\
Q&=\nonumber
\end{align}

\begin{align}
&\frac{1}{3} A+\frac{P}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} \left(3D-A^2\right)}{3 P}\nonumber\\
&\frac{1}{3} A-\frac{\left(1-i \sqrt{3}\right) P}{6 \sqrt[3]{2}}+\frac{\left(1+i \sqrt{3}\right) \left(3 D-A^2\right)}{3 \times 2^{2/3} P}\nonumber\\
&\frac{1}{3} A-\frac{\left(1+i \sqrt{3}\right) P}{6 \sqrt[3]{2}}+\frac{\left(1-i \sqrt{3}\right) \left(3D-A^2\right)}{3 \times 2^{2/3} P}\nonumber\\
&\frac{1}{3} B+\frac{\sqrt[3]{C+\sqrt{4 \left(3 \left(E\right)-(B)^2\right)^3+\left(C\right)^2}}}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} \left(3 \left(E\right)-(B)^2\right)}{3 \sqrt[3]{C+\sqrt{4 \left(3 \left(E\right)-(B)^2\right)^3+\left(C\right)^2}}}\nonumber\\
&\frac{1}{3} B-\frac{\left(1-i \sqrt{3}\right) \sqrt[3]{C+\sqrt{4 \left(3 \left(E\right)-(B)^2\right)^3+\left(C\right)^2}}}{6 \sqrt[3]{2}}+\frac{\left(1+i \sqrt{3}\right) \left(3 \left(E\right)-(B)^2\right)}{3 \times 2^{2/3} \sqrt[3]{C+\sqrt{4 \left(3 \left(E\right)-(B)^2\right)^3+\left(C\right)^2}}}\nonumber\\
&\frac{1}{3} B-\frac{\left(1+i \sqrt{3}\right) \sqrt[3]{C+\sqrt{4 \left(3 \left(E\right)-(Bf)^2\right)^3+\left(C\right)^2}}}{6 \sqrt[3]{2}}+\frac{\left(1-i \sqrt{3}\right) \left(3 \left(E\right)-(B)^2\right)}{3 \times 2^{2/3} \sqrt[3]{C+\sqrt{4 \left(3 \left(E\right)-(B)^2\right)^3+\left(C\right)^2}}}\nonumber
\end{align}

\begin{align}
&0=w^6\nonumber\\
&(-2 a -2 e-2 f)w^5\nonumber\\
&(+a^2 -b^2 -2 c^2 -2 d^2 +e^2 +f^2 -2 g^2 +4 a e +4 a f +4 e f )w^4\nonumber\\
&(+2 a c^2 +2 a d^2 -2 a e^2 -2 a f^2 -2 e f^2 +4 a g^2 +2 e g^2 +2 f g^2 -2 a^2 e +2 b^2 e +2 c^2 e \nonumber\\
&+4 d^2 e -2 a^2 f +2 b^2 f +4 c^2 f +2 d^2 f -2 e^2 f -8 a e f -4 c d g )w^3\nonumber\\
&(+c^4 +d^4 +g^4 +2 c^2 d^2 +a^2 e^2 -b^2 e^2 -2 d^2 e^2 +a^2 f^2 -b^2 f^2 -2 c^2 f^2 +e^2 f^2\nonumber\\
& +4 a e f^2 -2 a^2 g^2 +2 b^2 g^2 +2 c^2 g^2 +2 d^2 g^2 -4 a e g^2 -4 a f g^2 -2 e f g^2 -2 a c^2 e\nonumber\\
& -4 a d^2 e -4 a c^2 f -2 a d^2 f +4 a e^2 f +4 a^2 e f -4 b^2 e f -4 c^2 e f -4 d^2 e f +4 a c d g +4 c d e g +4 c d f g )w^2\nonumber\\
&(-2 a g^4 +4 c d g^3 +2 a d^2 e^2 +2 a c^2 f^2 -2 a e^2 f^2 -2 a^2 e f^2 +2 b^2 e f^2 +2 c^2 e f^2 -2 a c^2 g^2 -2 a d^2 g^2\nonumber\\
& +2 a^2 e g^2 -2 b^2 e g^2 -2 d^2 e g^2 +2 a^2 f g^2 -2 b^2 f g^2 -2 c^2 f g^2 +4 a e f g^2 -2 d^4 e -2 c^2 d^2 e -2 c^4 f \nonumber\\
&-2 c^2 d^2 f -2 a^2 e^2 f +2 b^2 e^2 f +2 d^2 e^2 f +4 a c^2 e f +4 a d^2 e f\nonumber\\
& +4 c d^3 g +4 c^3 d g -4 a c d e g -4 a c d f g -4 c d e f g) w\nonumber\\
&+a^2 g^4-b^2 g^4-4 a c d g^3+d^4 e^2+c^4 f^2+a^2 e^2 f^2-b^2 e^2 f^2-2 a c^2 e f^2\nonumber\\
&+4 c^2 d^2 g^2+2 a d^2 e g^2+2 a c^2 f g^2-2 a^2 e f g^2+2 b^2 e f g^2-2 a d^2 e^2 f+2 c^2 d^2 e f\nonumber\\
&-4 c d^3 e g-4 c^3 d f g+4 a c d e f g
\end{align}


\section{6x6 M1}
\begin{align}
A&=a+d-e+f+g+h\nonumber\\
B&=2 b^2+c^2+2 l^2+2 m^2+(n+p)^2+2 q^2-a d+a e-a f\nonumber\\
&-d f+e f-a g-d g+e g-f g-a h-d h+e h-g h\nonumber\\
C&=2 d b^2-2 e b^2+2 g b^2-4 c l b-4 n q b-4 p q b+2 a l^2+2 d l^2-2 e l^2\nonumber\\
&+2 a m^2+2 f m^2+2 h m^2+a n^2+g n^2+a p^2+g p^2+2 f q^2+2 g q^2\nonumber\\
&+2 h q^2+c^2 d-c^2 e+c^2 f-a d f+a e f-a d g+a e g-a f g-d f g\nonumber\\
&+e f g+c^2 h-a d h+a e h-a g h-d g h+e g h-4 l m n-4 l m p+2 a n p+2 g n p-4 c m q\nonumber\\
D&=4 m^2 b^2-2 d g b^2+2 e g b^2+4 c d l b-4 c e l b-4 c m n b-4 c m p b-8 l m q b\nonumber\\
&+4 g n q b+4 g p q b-2 a d l^2+2 a e l^2-2 a f m^2-2 a h m^2+c^2 n^2-a g n^2+c^2 p^2\nonumber\\
&-a g p^2+4 l^2 q^2-2 f g q^2-2 g h q^2-c^2 d f+c^2 e f+a d f g-a e f g-c^2 d h+c^2 e h\nonumber\\
&+a d g h-a e g h+4 a l m n+4 a l m p+2 c^2 n p-2 a g n p+4 c f m q+4 c h m q-4 c l n q-4 c l p q\nonumber\\
F&=d+e+f-h\,,\nonumber\\
G&=(d+e)( f-h)-(n-p)^2\nonumber
\end{align}
\begin{align}
P&=9ABC+72DB-2B^3+27(C^2+A^2 D)\nonumber\\
Q&=B^2-3AC+12D\nonumber\\
R&=\sqrt[3]{P+\sqrt{P^2-4 Q^3}}\nonumber\\
W&=\sqrt{\frac{1}{4}A^2+\frac{2}{3}B+\frac{R}{3 \sqrt[3]{2}}+\frac{\sqrt[3]{2} Q}{3 R}}\nonumber
\end{align}
\begin{align}
\omega_{1}^{2}&=\frac{1}{2} \left(F-\sqrt{F^2-4G}\right),\nonumber\\
\omega_{2}^{2}&=\frac{1}{2} \left(F+\sqrt{F^2-4G}\right),\nonumber\\
\omega_{3}^{2}&=\frac{1}{4}A-\frac{1}{2} W-\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-\frac{R}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} Q}{3 R}+\frac{A(4B+A^2)+8 C}{4W}}\,,\nonumber\\
\omega_{4}^{2}&=\frac{1}{4}A-\frac{1}{2} W+\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-\frac{R}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} Q}{3 R}+\frac{A(4B+A^2)+8 C}{4W}}\,,\nonumber\\
\omega_{5}^{2}&=\frac{1}{4}A+\frac{1}{2} W-\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-\frac{R}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} Q}{3 R}-\frac{A(4B+A^2)+8 C}{4W}}\,,\nonumber\\
\omega_{6}^{2}&=\frac{1}{4}A+\frac{1}{2} W+\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-\frac{R}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} Q}{3 R}-\frac{A(4B+A^2)+8 C}{4W}}\,,\nonumber
\end{align}
{\tiny 
\subsection{Autovalori in M1: autovettore V1}
\begin{align}
\Delta_{1}=(((2h-2f)l^2-gh^2+f^2g)q^2 +(c((2f-2h)lp+(2f-2h)ln+2h^2m-2f^2m) +b((2gh-2fg)p+(2gh-2fg)n+l(4fm-4hm))) q +a((fg-l^2)p^2+((2l^2-2gh)n+l(2hm-2fm))p+(fg-l^2)n^2 +l(2hm-2fm)n+f^2(m^2-dg)+h^2(dg-m^2) +(2df-2dh)l^2) +bc (2lp^2+(-4ln-2hm+2fm)p+2ln^2+(2fm-2hm)n +(4dh-4df)l) +b^2(-gp^2+2gnp-gn^2+h(2m^2-2dg)+f(2dg-2m^2)) +c^2(-fp^2+2hnp-fn^2-dh^2+df^2)),
\end{align}

\begin{align}
x_1&=\frac{ -(((2l^2-gh-fg)(p-n) +2(d+e)(h-)fl^2 +(d+ e)g(f^2-h^2) q +c(-lp^3+(ln+hm+fm)p^2 +(ln^2+(-2hm-2fm)n+((-d- e)h+(d+ e)f)l)p-ln^3 +(hm+fm)n^2+((-d- e)h+(d+ e)f)ln+(d+ e)h^2m +(-d- e)f^2m) +b(gp^3+(-gn-2lm)p^2+(-gn^2+4lmn+(d+ e)gh+(-d- e)fg)p +gn^3-2lmn^2+((d+ e)gh+(-d- e)fg)n +l((-2d-2 e)hm+(2d+2 e)fm)))}{\Delta_{1}}\nonumber\\
x_2&= \frac{-(((2l^2-gh-fg)p+(-2l^2+gh+fg)n)q^2 +(c(-3lp^2+(2ln+2hm+2fm)p+ln^2+(-2hm-2fm)n +((-d- e)h+(d+ e)f)l) +b(3gp^2+(-2gn-4lm)p-gn^2+4lmn+(d+ e)gh+(-d- e)fg)) q +a(-gp^3+3lmp^2 +(gn^2-2lmn+f(dg-m^2)+h(-m^2- eg)+( e-d)l^2)p -lmn^2+(h(m^2-dg)+f(m^2+ eg)+(d- e)l^2)n +l((d+ e)hm+(-d- e)fm)) +c^2(p^3+(-n^2+ eh-df)p+(dh- ef)n) +bc (-3mp^2+(2mn+(2d-2 e)l)p+mn^2+(2 e-2d)ln+(-d- e)hm +(d+ e)fm) +b^2((2m^2+( e-d)g)p+((d- e)g-2m^2)n))}{\Delta-{1}}, \nonumber\\
x_3&= \frac{(((2l^2-gh-fg)p+(-2l^2+gh+fg)n)q^2 +(c(-lp^2+(-2ln+2hm+2fm)p+3ln^2+(-2hm-2fm)n +((d+ e)h+(-d- e)f)l) +b(gp^2+(2gn-4lm)p-3gn^2+4lmn+(-d- e)gh+(d+ e)fg)) q +a((lm-gn)p^2+(2lmn+h(dg-m^2)+f(-m^2- eg)+( e-d)l^2)p +gn^3-3lmn^2 +(f(m^2-dg)+h(m^2+ eg)+(d- e)l^2)n +l((-d- e)hm+(d+ e)fm)) +c^2(np^2+( ef-dh)p-n^3+(df- eh)n) +bc (-mp^2+((2d-2 e)l-2mn)p+3mn^2+(2 e-2d)ln+(d+ e)hm +(-d- e)fm)+b^2((2m^2+( e-d)g)p+((d- e)g-2m^2)n))}{\Delta_{1}}, \nonumber\\
x_4&= \frac{-((b(-2lp^2+4lnp-2ln^2+((-2d-2 e)h+(2d+2 e)f)l) +c((h+f)p^2+(-2h-2f)np+(h+f)n^2+(d+ e)h^2+(-d- e)f^2)) q +a(lp^3+(-ln-hm-fm)p^2 +(-ln^2+(2hm+2fm)n+((d+ e)h+(-d- e)f)l)p+ln^3 +(-hm-fm)n^2+((d+ e)h+(-d- e)f)ln+(-d- e)h^2m +(d+ e)f^2m) +bc (-p^3+np^2+(n^2+(-d- e)h+(d+ e)f)p-n^3 +((-d- e)h+(d+ e)f)n) +b^2(2mp^2-4mnp+2mn^2+(2d+2 e)hm+(-2d-2 e)fm))}{(((2h-2f)l^2-gh^2+f^2g)q^2 +(c((2f-2h)lp+(2f-2h)ln+2h^2m-2f^2m) +b((2gh-2fg)p+(2gh-2fg)n+l(4fm-4hm))) q +a((fg-l^2)p^2+((2l^2-2gh)n+l(2hm-2fm))p+(fg-l^2)n^2 +l(2hm-2fm)n+f^2(m^2-dg)+h^2(dg-m^2) +(2df-2dh)l^2) +bc (2lp^2+(-4ln-2hm+2fm)p+2ln^2+(2fm-2hm)n +(4dh-4df)l) +b^2(-gp^2+2gnp-gn^2+h(2m^2-2dg)+f(2dg-2m^2)) +c^2(-fp^2+2hnp-fn^2-dh^2+df^2))}, \nonumber\\
x_5&=\frac{ (((2h-2f)l^2-gh^2+f^2g)q^2 +(c((2f-2h)lp+(2f-2h)ln+2h^2m-2f^2m) +b((2gh-2fg)p+(2gh-2fg)n+l(4fm-4hm))) q +a((l^2-gh)p^2+((2fg-2l^2)n+l(2hm-2fm))p+(l^2-gh)n^2 +l(2hm-2fm)n+f^2(m^2+ eg)+h^2(-m^2- eg) +(2 eh-2 ef)l^2) +bc (-2lp^2+(4ln-2hm+2fm)p-2ln^2+(2fm-2hm)n +(4 ef-4 eh)l) +c^2(hp^2-2fnp+hn^2+ eh^2- ef^2) +b^2(gp^2-2gnp+gn^2+h(2m^2+2 eg)+f(-2m^2-2 eg)))}{(((2h-2f)l^2-gh^2+f^2g)q^2 +(c((2f-2h)lp+(2f-2h)ln+2h^2m-2f^2m) +b((2gh-2fg)p+(2gh-2fg)n+l(4fm-4hm))) q +a((fg-l^2)p^2+((2l^2-2gh)n+l(2hm-2fm))p+(fg-l^2)n^2 +l(2hm-2fm)n+f^2(m^2-dg)+h^2(dg-m^2) +(2df-2dh)l^2) +bc (2lp^2+(-4ln-2hm+2fm)p+2ln^2+(2fm-2hm)n +(4dh-4df)l) +b^2(-gp^2+2gnp-gn^2+h(2m^2-2dg)+f(2dg-2m^2)) +c^2(-fp^2+2hnp-fn^2-dh^2+df^2))}\nonumber\\
x_6&=1\nonumber
\end{align}
}

\section{6x6 M2}
\begin{align}
A&=a+b+e+f\nonumber\\
B&=a-b+e+f\nonumber\\
C_{1}&=2 a^3+6 b a^2-3 e a^2-3 f a^2+6 b^2 a+9 c^2 a+9 d^2 a-3 e^2 a-3 f^2 a-18 g^2 a-18 h^2 a+9 m^2 a+9 n^2 a-6 b e a-6 b f a+12 e f a+2 b^3+2 e^3+2 f^3+9 b c^2+9 b d^2-3 b e^2-3 b f^2-3 e f^2-18 b g^2+9 e g^2+9 f g^2-18 b h^2+9 e h^2+9 f h^2+9 b m^2+9 e m^2-18 f m^2+9 b n^2-18 e n^2+9 f n^2-3 b^2 e+9 c^2 e-18 d^2 e-3 b^2 f-18 c^2 f+9 d^2 f-3 e^2 f+12 b e f+54 c d g+54 d h m-54 c h n+54 g m n\nonumber\\
C_{2}&=2 a^3-6 b a^2-3 e a^2-3 f a^2+6 b^2 a+9 c^2 a+9 d^2 a-3 e^2 a-3 f^2 a-18 g^2 a-18 h^2 a+9 m^2 a+9 n^2 a+6 b e a+6 b f a+12 e f a-2 b^3+2 e^3+2 f^3-9 b c^2-9 b d^2+3 b e^2+3 b f^2-3 e f^2+18 b g^2+9 e g^2+9 f g^2+18 b h^2+9 e h^2+9 f h^2-9 b m^2+9 e m^2-18 f m^2-9 b n^2-18 e n^2+9 f n^2-3 b^2 e+9 c^2 e-18 d^2 e-3 b^2 f-18 c^2 f+9 d^2 f-3 e^2 f-12 b e f+54 c d g+54 d h m-54 c h n+54 g m n\nonumber
D&=-c^2-d^2-g^2-h^2-m^2-n^2+a e+b e+a f+b f+e f\nonumber\\
E&=c^2-d^2-g^2-h^2-m^2-n^2+a e-b e+a f-b f+e f\nonumber
\end{align}

B
CDCC1

\begin{align}
&\frac{1}{3} A+\frac{\sqrt[3]{C+\sqrt{4 \left(3 \left(D\right)-A^2\right)^3+\left(C\right)^2}}}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} \left(3 \left(D\right)-A^2\right)}{3 \sqrt[3]{C+\sqrt{4 \left(3 \left(D\right)-A^2\right)^3+\left(C\right)^2}}}\nonumber\\
&\frac{1}{3} A-\frac{\left(1-i \sqrt{3}\right) \sqrt[3]{C+\sqrt{4 \left(3 \left(D\right)-A^2\right)^3+\left(C\right)^2}}}{6 \sqrt[3]{2}}+\frac{\left(1+i \sqrt{3}\right) \left(3 \left(D\right)-A^2\right)}{3 \times 2^{2/3} \sqrt[3]{C+\sqrt{4 \left(3 \left(D\right)-A^2\right)^3+\left(C\right)^2}}}\nonumber\\
&\frac{1}{3} A-\frac{\left(1+i \sqrt{3}\right) \sqrt[3]{C+\sqrt{4 \left(3 \left(D\right)-A^2\right)^3+\left(C\right)^2}}}{6 \sqrt[3]{2}}+\frac{\left(1-i \sqrt{3}\right) \left(3 \left(D\right)-A^2\right)}{3 \times 2^{2/3} \sqrt[3]{C+\sqrt{4 \left(3 \left(D\right)-A^2\right)^3+\left(C\right)^2}}}\nonumber\\
&\frac{1}{3} B+\frac{\sqrt[3]{C1+\sqrt{4 \left(3 \left(-E\right)--B^2\right)^3+\left(C1\right)^2}}}{3 \sqrt[3]{2}}-\frac{\sqrt[3]{2} \left(3 \left(-E\right)--B^2\right)}{3 \sqrt[3]{C1+\sqrt{4 \left(3 \left(-E\right)--B^2\right)^3+\left(C1\right)^2}}}\nonumber\\
&\frac{1}{3} B-\frac{\left(1-i \sqrt{3}\right) \sqrt[3]{C1+\sqrt{4 \left(3 \left(-E\right)--B^2\right)^3+\left(C1\right)^2}}}{6 \sqrt[3]{2}}+\frac{\left(1+i \sqrt{3}\right) \left(3 \left(-E\right)--B^2\right)}{3 \times 2^{2/3} \sqrt[3]{C1+\sqrt{4 \left(3 \left(-E\right)--B^2\right)^3+\left(C1\right)^2}}}\nonumber\\
&\frac{1}{3} B-\frac{\left(1+i \sqrt{3}\right) \sqrt[3]{C1+\sqrt{4 \left(3 \left(-E\right)--B^2\right)^3+\left(C1\right)^2}}}{6 \sqrt[3]{2}}+\frac{\left(1-i \sqrt{3}\right) \left(3 \left(-E\right)--B^2\right)}{3 \times 2^{2/3} \sqrt[3]{C1+\sqrt{4 \left(3 \left(-E\right)--B^2\right)^3+\left(C1\right)^2}}}
\end{align}


CALCOLI C1 e C2 per M2

\begin{align}
C_{1}&=2 a^3+3 a^2(b-e-f)\nonumber\\
&+3a(2b^2+3(c^2+d^2)-e^2 -f^2 -6(g^2+h^2) +3(m^2 +n^2)-2b(e+f)+6ef)\nonumber\\
&+2 (b^3+e^3+ f^3)+3b(c^2+3 d^2- e^2-f^2)+9(g^2+h^2)(-2b+e+f)\nonumber\\
&+9m^2(b+e-3f)+9n^2(b+f-3e)-3e(b^2+f^2-3c^2+6d^2)\nonumber\\
&-3f(b^2+6c^2-3d^2+e^2+4b e)+54(c d g+d h m-c h n+ g m n)\nonumber\\
C_{2}&=2 a^3-3a^2(b+e+f)\nonumber\\
&+3a(2b^2+3(c^2+d^2)-e^2 -f^2 -6(g^2+h^2) +3(m^2 +n^2)+2b(e+f)+6ef)\nonumber\\
&-2(b^3-e^3-f^3)-3b(c^2+d^2-e^2-f^2)+9(g^2+h^2)(2b+e f)\nonumber\\
&-9m^2(b-e+3f)-9n^2(b-f+3e)-3e(b^2+f^2-3c^2+6d^2)\nonumber\\
&-3f(b^2+6c^2-3d^2+e^2-4b e)+54(c d g+d h m-c h n+g m n)\nonumber
\end{align}

CALCOLI C1 e C2 per N3=M2 (m=n=h=0)

\begin{align}
C_{1}&=2 a^3+3 a^2(b-e-f)\nonumber\\
&+3a(2b^2+3(c^2+d^2)-e^2 -f^2 -6g^2 -2b(e+f)+6ef)\nonumber\\
&+2 (b^3+e^3+ f^3)+3b(c^2+3 d^2- e^2-f^2)+9g^2(-2b+e+f)\nonumber\\
&-3e(b^2+f^2-3c^2+6d^2)-3f(b^2+6c^2-3d^2+e^2+4b e)+54c d g\nonumber\\
C_{2}&=2 a^3-3a^2(b+e+f)\nonumber\\
&+3a(2b^2+3(c^2+d^2)-e^2 -f^2 -6g^2 +2b(e+f)+6ef)\nonumber\\
&-2(b^3-e^3-f^3)-3b(c^2+d^2-e^2-f^2)+9g^2(2b+e+f)\nonumber\\
&-3e(b^2+f^2-3c^2+6d^2)-3f(b^2+6c^2-3d^2+e^2-4b e)+54c d g\nonumber\\
\end{align}


\begin{align}
A&=(a+d-e+f+g+h)\,,\nonumber\\
%
B&=2b^2+c^2+2 l^2+2 m^2+n^2+p^2+2 q^2-a d+a e-a f-d f+e f-a g-d g+e g-f g-a h-d h+e h-g h+2 n p\,,\nonumber\\
%
C&=2 d b^2-2 e b^2+2 g b^2-4 c l b-4 n q b-4 p q b+2 a l^2+2 d l^2-2 e l^2+2 a m^2+2 f m^2+2 h m^2+a n^2+g n^2+a p^2+g p^2+2 f q^2+2 g q^2+2 h q^2+c^2 d-c^2 e+c^2 f-a d f+a e f-a d g+a e g-a f g-d f g+e f g+
c^2 h-a d h+a e h-a g h-d g h+e g h-4 l m n-4 l m p+2 a n p+2 g n p-4 c m q\,,\nonumber\\
%
D&=4 m^2 b^2-2 d g b^2+2 e g b^2+4 c d l b-4 c e l b-4 c m n b-4 c m p b-8 l m q b+4 g n q b+4 g p q b-2 a d l^2+2 a e l^2-2 a f m^2-2 a h m^2+c^2 n^2-a g n^2+c^2 p^2-a g p^2+4 l^2 q^2-2 f g q^2-2 g h q^2-c^2 d f+c^2 e f+a d f g-a e f g-c^2 d h+c^2 e h+a d g h-a e g h+4 a l m n+4 a l m p+2 c^2 n p-2 a g n p+4 c f m q+4 c h m q-4 c l n q-4 c l p q\,,\nonumber\\
%
P&=-2B^3-9ACB+72DB+27 C^2+27 A^2 D\,,\nonumber\\
%
Q&=B^2+3AC+12 D\,,\nonumber\\
%
S&=A^3+4AB-8 C\,,\nonumber\\
%
W&=\frac{\sqrt[3]{P+\sqrt{P^2-4Q^3}}}{3 \sqrt[3]{2}}+\frac{\sqrt[3]{2} Q}{3 \sqrt[3]{P+\sqrt{P^2-4Q^3}}}\,,\nonumber\\
\end{align}

\begin{align}
\omega_{3}^{2}&=\frac{1}{4}A -\frac{1}{2} \sqrt{\frac{1}{4} A^2+\frac{2}{3}B+W}-\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-W-\frac{S}{4 \sqrt{\frac{1}{4} A^2+\frac{2}{3}B+W}}}\,,\nonumber\\
%
\omega_{4}^{2}&=\frac{1}{4}A -\frac{1}{2} \sqrt{\frac{1}{4} A^2+\frac{2}{3}B+W}+\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-W-\frac{S}{4 \sqrt{\frac{1}{4} A^2+\frac{2}{3}B+W}}}\,,\nonumber\\
%
\omega_{5}^{2}&=\frac{1}{4}A +\frac{1}{2} \sqrt{\frac{1}{4} A^2+\frac{2}{3}B+W}-\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-W+\frac{S}{4 \sqrt{\frac{1}{4} A^2+\frac{2}{3} B+W}}}\,,\nonumber\\
%
\omega_{6}^{2}&=\frac{1}{4}A+\frac{1}{2} \sqrt{\frac{1}{4} A^2+\frac{2}{3}B+W}+\frac{1}{2} \sqrt{\frac{1}{2} A^2+\frac{4}{3}B-W+\frac{S}{4 \sqrt{\frac{1}{4} A^2+\frac{2}{3} B+W}}}\,,\nonumber
\end{align}





==> leftovers/eigen.tex <==
\section{The eigenvectors for the micromorphic propagation condition}

\subsection{The eigenvectors in the subspace $\caN_{3}$}

Ricordarsi che $c$ e $d$ vanno messi complessi coniugati e che bisogna sostituire ad $a$ $a-\omega^{2}$ ecc.


\begin{itemize}
\item
$w_{1}=\{\alpha_{1}\,,\beta_{1}\,,\gamma_{1}\,,\delta_{1}\,,\epsilon_{1}\,,1\}$
\begin{align}
\alpha_{1}&=-\frac{dg(a(g^2- ef)+3c^2f)+acf( ef-g^2) +cd^2(-2g^2- ef)+ ed^3g -c^3f^2 }{\Delta}\,,\nonumber\\ 
\beta_{1} &=\frac{b (d(g^3- efg)+c( ef^2-fg^2)) }{\Delta}\,,\nonumber\\ 
\gamma_{1} &=-\frac{b(d^2g^2-2cdfg+c^2f^2) }{\Delta}\,,\nonumber\\ 
\delta_{1} &=\frac{(a^2-b^2)(g^3- efg)-d(ac(3g^2- ef)+c^3f+d^2g(2c^2+ea)+ac^2fg+ ecd^3}{\Delta}\,,\nonumber\\ 
\epsilon_{1} &=\frac{ b(g(c^2f+ ed^2)-cd(g^2+ef)) }{\Delta}\,,\nonumber
\end{align}
where
\begin{align}
\Delta&=d^2(a(g^2-2 ef)+c^2f)+f(b^2-a^2)(g^2- ef)+2acdfg-2cd^3g-ac^2f^2 + ed^4\,.\nonumber
\end{align}
\item
$w_{2}=\{\alpha_{2}\,,\beta_{2}\,,\gamma_{2}\,,\delta_{2}\,,1\,,\theta_{2}\}$
\begin{align}
\alpha_{2} &=\frac{b(ed-cg)( ef-g^2)}{\Delta}\,,\nonumber\\ 
\beta_{2} &=\frac{a(cg-de)( ef-g^2)+dc^2(2g^2+ ef)-c^3fg -3 ecd^2g+ e^2d^3}{\Delta}\,,\nonumber\\ 
\gamma_{2} &=\frac{g(a^2-b^2)(g^2- ef)-d(ac(3g^2- ef)+c^3f)-d^2(-2c^2g- eag)+ac^2fg-ecd^3}{\Delta}\,,\nonumber\\ 
\delta_{2} &=-\frac{b(c^2g^2-2 ecdg+ e^2d^2) }{\Delta}\,,\nonumber\\ 
\theta_{2} &=\frac{ b(g(c^2f+ ed^2)-cd(g^2+ef)) }{\Delta}\,,\nonumber
\end{align}
where
\begin{align}
\Delta&=e(b^2-a^2)(g^2- ef)+ac^2(g^2-2 ef)+cdg(2 ea-2c^2)+c^4f +( c^2- ea)ed^2\,.\nonumber
\end{align}
\item
$w_{3}=\{\alpha_{3}\,,\beta_{3}\,,\gamma_{3}\,,1\,,\epsilon_{3}\,,\theta_{3}\}$
\begin{align}
\alpha_{3}&=\frac{ a(g^2-cf)+c^2(d-g)}{d(c^2-ag)-bc^2}\,,\nonumber\\ 
\beta_{3} &=\frac{ g(d^2-bg)+fc(b-d)}{d(c^2-ag)-bc^2}\,,\nonumber\\ 
\gamma_{3} &=\frac{e(g^2-cf)(b^2-a^2)+ac^2g(g+e)-d(ac^2- ebcf-c^4)-ac^3f-ebd^2g-c^4g}{(cg-ed)(d(ag-c^2)+bc^2)\,,}\nonumber\\ 
\epsilon_{3}&=\frac{ bcg+adf-cd^2}{d(c^2-ag)-bc^2}\,,\nonumber\\ 
\theta_{3} &=\frac{(g^3-cfg)(a^2-b^2)-dc(g(ag+bf)+c(cg-af-ag))-d^2(c^3-bg^2)-ac^2g^2}{(cg-ed)(d(ag-c^2)+bc^2)}\,.\nonumber
\end{align}


\item
$w_{4}=\{\alpha_{4}\,,\beta_{4}\,,1\,,\delta_{4}\,,\epsilon_{4}\,,\theta_{4}\}$
\begin{align}
\alpha_{4}&=\frac{b(dg-cf)(g^2- ef)}{\Delta}\,,\nonumber\\ 
\beta_{4}&=\frac{a(cf-dg)(g^2- ef)+cd^2(2g^2+ef)-3dgc^2f-d^3g+c^3f^2}{\Delta}\,,\nonumber\\
\delta_{4}&=\frac{ b(g(c^2f+ ed^2)-cd(g^2+ef)) }{\Delta}\,,\nonumber\\ 
\epsilon_{4}&=\frac{g(a^2-b^2)(g^2- ef)-d(ac(3g^2- ef)-c^3f)+gd^2(2c^2+ea)+ac^2fg-ecd^3}{\Delta}\,,\nonumber\\ 
\theta_{4}&=-\frac{b(dg-cf)^2 }{\Delta}\,,\nonumber
\end{align}
where
\begin{align}
\Delta&=d^2(a(g^2-2 ef)+c^2f)+f(a^2-b^2)( ef-g^2) +2cdg(af-d^2)-ac^2f^2 + ed^4\,.\nonumber
\end{align}
\item
$w_{5}=\{\alpha_{5}\,,1\,,\gamma_{5}\,,\delta_{5}\,,\epsilon_{5}\,,\theta_{5}\}$
\begin{align}
\alpha_{5} &=\frac{b(ef-g^2)}{a(g^2- ef)-2cdg+c^2f+ ed^2}\,,\nonumber\\
\gamma_{5}&=\frac{ cf-dg}{g^2- ef}\,, \nonumber\\
\delta_{5} &=\frac{ -b( ed-cg)}{a(g^2- ef)-2cdg+c^2f+ ed^2}\,, \nonumber\\
\epsilon_{5} &=\frac{ed-cg}{g^2- ef}\,, \nonumber\\
\theta_{5} &=\frac{ b(bg-cf)}{a(g^2- ef)-2cdg+c^2f+ ed^2}\,.\nonumber
\end{align}
\item
$w_{6}=\{1\,,\beta_{6}\,,\gamma_{6}\,,\delta_{6}\,,\epsilon_{6}\,,\theta_{6}\}$
\begin{align}
\beta_{6} &=\alpha_{5}\,,\quad\delta_{6}=\epsilon_{5}\,,\quad\epsilon_{6}=\delta_{5}\,,\quad\theta_{6}=\gamma_{5}\,,\\
\gamma_{6} &=\frac{ b(dg-cf)}{a(g^2- ef)-2cdg+c^2f+ ed^2}\,. \nonumber
\end{align}
\end{itemize}

\subsection{The eigenvectors in the subspace $\caM_{1}$}

\subsubsection{$w_{1}=\{\alpha_{1}\,,\beta_{1}\,,\gamma_{1}\,,\delta_{1}\,,\epsilon_{1}\,,1\}$}

All the components must be divided by:
\begin{align}
\Delta&=(((2h-2f)l^2-gh^2+f^2g)q^2 +(c((2f-2h)lp+l(fn-hn)+((f-h)l+2h^2-2f^2)m) +b((2gh-2fg)p+ghn-fgn+((4f-4h)l+gh-fg)m)) q +a((fg-l^2)p^2+(l^2n-ghn+(l^2+(2h-2f)l-gh)m)p +m(l(hn-fn)-l^2n+fgn)+((h-f)l-h^2+f^2)m^2 +(2df-2dh)l^2+dgh^2-df^2g) +bc (2lp^2+((-2l-2h+2f)m-2ln)p+m(2ln-hn+fn)+(f-h)m^2 +(4dh-4df)l) +b^2(-gp^2+(gn+gm)p-gmn+(2h-2f)m^2-2dgh+2dfg) +c^2(-fp^2+(hn+hm)p-fmn-dh^2+df^2))\,.\nonumber
\end{align}

\begin{align}
A&=2l^2-g(h+f)\nonumber\\
B&=\nonumber\\
C&=\nonumber\\
D&=\nonumber\\
E&=\nonumber\\
F&=\nonumber\\
G&=\nonumber\\
H&=\nonumber
\end{align}

\begin{align}
\alpha_{1}&=\frac{-1}{\Delta}((Ap^2+(-3l^2n+ghn+2fgn+(gh-l^2)m)p +l^2(n^2+(d+e)h-2(d+e)f) -ghn^2+m(l(hn-fn)+l^2n-fgn) +(f-h)lm^2+(-d- e)gh^2+(d+ e)f^2g) q +c(-lp^3+(ln+(h+f)m)p^2 +(m(ln-hn-2fn)-hm^2+((-d- e)h+(d+ e)f)l)p +m(hn^2+l(-n^2- eh+ ef)+(d+ e)h^2+(-d- e)f^2) +l(dfn-dhn)+fm^2n) +b(gp^3+(-gn-2lm)p^2 +(m(3ln-gn)+lm^2+(d+ e)gh+(-d- e)fg)p +m(gn^2+l(-n^2+(-2d-2 e)h+(2d+2 e)f)+ egh - efg)+m^2(-ln-hn+fn)+dghn-dfgn +(h-f)m^3)) \nonumber\\ 
\beta_{1}&=\frac{-1}{\Delta}((Ap-l^2n+ghn+(fg-l^2)m)q^2 +(c(-3lp^2+(ln+(l+2h+2f)m)p+m(ln-2hn)-2fm^2 +((-d- e)h+(d+ e)f)l) +b(3gp^2+((-4l-g)m-gn)p+m(2ln-gn)+2lm^2+(d+ e)gh +(-d- e)fg)) q +a(-gp^3+3lmp^2 +(m(gn-ln)+(-l-h-f)m^2+( e-d)l^2- egh+dfg)p +m^2(hn-ln)+dl^2n-dghn+fm^3 +(- el^2+((d+ e)h+(-d- e)f)l+ efg)m) +c^2(p^3+(-mn+ eh-df)p+dhn- efm) +bc (-3mp^2+(mn+m^2+(2d-2 e)l)p+m^2n-2dln +(2 el+(-d- e)h+(d+ e)f)m) +b^2((2m^2+( e-d)g)p-m^2n+dgn-m^3- egm)) \nonumber\\ 
\gamma_{1}&=\frac{1}{\Delta} ((Ap-l^2n+fgn+(gh-l^2)m)q^2 +(c(-lp^2+((2h+2f)m-2ln)p+l(n^2+(d+ e)h+(-d- e)f) +m(2ln-2fn)-2hm^2) +b(gp^2+(2gn-4lm)p-gn^2+m(2ln-2gn)+2lm^2+(-d- e)gh +(d+ e)fg)) q +a((lm-gn)p^2+(2lmn+(-h-f)m^2+( e-d)l^2+dgh- efg)p +m(gn^2+l(-n^2+(-d- e)h+(d+ e)f)- el^2 + egh)+m^2(fn-2ln)+dl^2n-dfgn +hm^3) +c^2(np^2+( ef-dh)p+m(-n^2- eh)+dfn) +bc (-mp^2+((2d-2 e)l-2mn)p+m(n^2+2 el+(d+ e)h+(-d- e)f) +2m^2n-2dln) +b^2((2m^2+( e-d)g)p-m^2n+dgn-m^3- egm))\nonumber\\ 
\delta_{1}&=\frac{-1}{\Delta}((l(fn-hn)+(h-f)lm)q^2 +(b(-2lp^2+(3ln+lm)p+l(-n^2+(-2d-2 e)h+(2d+2 e)f) +m(-ln+hn-fn)+(f-h)m^2) +c((h+f)p^2+(-hn-2fn-hm)p+hn^2+fmn+(d+ e)h^2 +(-d- e)f^2)) q +a(lp^3+((-h-f)m-ln)p^2 +(m(-ln+hn+2fn)+hm^2+((d+ e)h+(-d- e)f)l)p +m(l(n^2+ eh- ef)-hn^2+(-d- e)h^2+(d+ e)f^2) +l(dhn-dfn)-fm^2n) +bc (-p^3+np^2+(mn+(-d- e)h+(d+ e)f)p+m(-n^2- eh+ ef)-dhn +dfn) +b^2(2mp^2+(-3mn-m^2)p+m(n^2+(2d+2 e)h+(-2d-2 e)f) +m^2n)) \nonumber\\ 
\epsilon_{1}&=\frac{1}{\Delta} (((2h-2f)l^2-gh^2+f^2g)q^2 +(c((2f-2h)lp+l(2fn-2hn)+(2h^2-2f^2)m) +b((2gh-2fg)p+2ghn-2fgn+(4f-4h)lm)) q +a((l^2-gh)p^2+(-2l^2n+2fgn+(2h-2f)lm)p +l^2(n^2+2 eh-2 ef)-ghn^2+lm(2hn-2fn) +(f^2-h^2)m^2- egh^2+ ef^2g) +bc (-2lp^2+(4ln+(2f-2h)m)p+l(-2n^2-4 eh+4 ef) +m(2fn-2hn)) +c^2(hp^2-2fnp+hn^2+ eh^2- ef^2) +b^2(gp^2-2gnp+gn^2+(2h-2f)m^2+2 egh-2 efg)) \nonumber\\
\theta_{1}&=1\nonumber
\end{align}

\subsubsection{$\Vb_{2}$}
\begin{align}
\Delta&=(((2h-2f)l^2-gh^2+f^2g)q^2 +a((l^2-fg)p^2+((2gh-2l^2)n+l(2fm-2hm))p+(l^2-fg)n^2 +l(2fm-2hm)n+h^2(m^2-dg)+f^2(dg-m^2) +(2dh-2df)l^2) +bc (-2lp^2+(4ln+2hm-2fm)p-2ln^2+(2hm-2fm)n +(4df-4dh)l) +b^2(gp^2-2gnp+gn^2+f(2m^2-2dg)+h(2dg-2m^2)) +c^2(fp^2-2hnp+fn^2+dh^2-df^2))\nonumber
\end{align}

\begin{align}
A&=(2l^2-gh-fg)\nonumber\\
B&=\nonumber\\
C&=\nonumber\\
D&=\nonumber\\
E&=\nonumber\\
F&=\nonumber\\
G&=\nonumber\\
H&=\nonumber
\end{align}

\begin{align}
\alpha&=\frac{ -((Ap^2+(-4l^2+2gh+2fg)np +An^2 +((2d+2 e)h+(-2d-2 e)f)l^2 +(-d- e)gh^2+(d+ e)f^2g) q +c(-lp^3+(ln+hm+fm)p^2 +(ln^2+(-2hm-2fm)n+((-d- e)h+(d+ e)f)l)p-ln^3 +(hm+fm)n^2+((-d- e)h+(d+ e)f)ln+(d+ e)h^2m +(-d- e)f^2m) +b(gp^3+(-gn-2lm)p^2+(-gn^2+4lmn+(d+ e)gh+(-d- e)fg)p +gn^3-2lmn^2+((d+ e)gh+(-d- e)fg)n +l((-2d-2 e)hm+(2d+2 e)fm))) }{\Delta}\nonumber\\ 
\beta&=\frac{ -((Ap+(-2l^2+gh+fg)n)q^2 +(c(-lp^2+2lnp-ln^2+((-d- e)h+(d+ e)f)l) +b(gp^2-2gnp+gn^2+(d+ e)gh+(-d- e)fg)) q +a((gn-lm)p^2+(-2lmn+h(m^2-dg)+f(m^2+ eg)+(d- e)l^2)p -gn^3+3lmn^2 +(f(dg-m^2)+h(-m^2- eg)+( e-d)l^2)n +l((d+ e)hm+(-d- e)fm)) +c^2(-np^2+(dh- ef)p+n^3+( eh-df)n) +bc (mp^2+(2mn+(2 e-2d)l)p-3mn^2+(2d-2 e)ln+(-d- e)hm +(d+ e)fm)+b^2(((d- e)g-2m^2)p+(2m^2+( e-d)g)n)) }{\Delta}\nonumber\\ 
\gamma&=\frac{ ((Ap+(-2l^2+gh+fg)n)q^2 +(c(lp^2-2lnp+ln^2+((d+ e)h+(-d- e)f)l) +b(-gp^2+2gnp-gn^2+(-d- e)gh+(d+ e)fg)) q +a(gp^3-3lmp^2 +(-gn^2+2lmn+f(m^2-dg)+h(m^2+ eg)+(d- e)l^2)p +lmn^2+(h(dg-m^2)+f(-m^2- eg)+( e-d)l^2)n +l((-d- e)hm+(d+ e)fm)) +c^2(-p^3+(n^2- eh+df)p+( ef-dh)n) +bc (3mp^2+((2 e-2d)l-2mn)p-mn^2+(2d-2 e)ln+(d+ e)hm +(-d- e)fm) +b^2(((d- e)g-2m^2)p+(2m^2+( e-d)g)n)) }{\Delta}\nonumber\\ 
\delta&=\frac{ -((b(-2lp^2+4lnp-2ln^2+((-2d-2 e)h+(2d+2 e)f)l) +c((h+f)p^2+(-2h-2f)np+(h+f)n^2+(d+ e)h^2+(-d- e)f^2)) q +a(lp^3+(-ln-hm-fm)p^2 +(-ln^2+(2hm+2fm)n+((d+ e)h+(-d- e)f)l)p+ln^3 +(-hm-fm)n^2+((d+ e)h+(-d- e)f)ln+(-d- e)h^2m +(d+ e)f^2m) +bc (-p^3+np^2+(n^2+(-d- e)h+(d+ e)f)p-n^3 +((-d- e)h+(d+ e)f)n) +b^2(2mp^2-4mnp+2mn^2+(2d+2 e)hm+(-2d-2 e)fm)) }{\Delta}\nonumber\\ 
\epsilon&=1\nonumber\\
\theta&=\frac{ (((2h-2f)l^2-gh^2+f^2g)q^2 +a((gh-l^2)p^2+((2l^2-2fg)n+l(2fm-2hm))p+(gh-l^2)n^2 +l(2fm-2hm)n+h^2(m^2+ eg)+f^2(-m^2- eg) +(2 ef-2 eh)l^2) +bc (2lp^2+(-4ln+2hm-2fm)p+2ln^2+(2hm-2fm)n +(4 eh-4 ef)l) +c^2(-hp^2+2fnp-hn^2- eh^2+ ef^2) +b^2(-gp^2+2gnp-gn^2+f(2m^2+2 eg)+h(-2m^2-2 eg))) }{\Delta}\nonumber
\end{align}

\subsubsection{$\Vb_{3}$}
\begin{align}
\Delta&=(2h+2(f-\omega^{2}))q^2+b(-4p-4n)q+(a-\omega^{2})(p^2+2np+n^2+( e-(d-\omega^{2}))h\nonumber\\
&+( e-(d-\omega^{2}))(f-\omega^{2})) +b^2(2(d-\omega^{2})-2 e)\nonumber
\end{align}
\begin{align}
A&=(2lp+2ln-2hm-2(f-\omega^{2})m)\nonumber\\
B&=(-p^2-2np-n^2+((d-\omega^{2})- e)h+((d-\omega^{2})- e)(f-\omega^{2}))\nonumber\\
C&=(2mp+2mn+(2 e-2(d-\omega^{2}))\nonumber\\
D&=(2lq^2+(c(-p-n)-2bm)\nonumber\\
E&=(mp+mn+( e-(d-\omega^{2}))l)\nonumber\\
F&=(d-\omega^{2})-e\nonumber\\
G&=(c(h+(f-\omega^{2}))-2bl)\nonumber\\
H&=(lp+ln-hm-(f-\omega^{2})m)\nonumber\\
L&=(-p-n)\nonumber
\end{align}
\begin{align}
\alpha&=\frac{qA+cB +bC}{\Delta}\nonumber\\
\beta&=\gamma=\frac{-Dq+(a-\omega^{2})E+bcF}{\Delta} \nonumber\\
\delta&=1 \nonumber\\
\epsilon&=-\theta=-\frac{(Gq+(a-\omega^{2})H+bcL+2b^2m)}{\Delta} \nonumber
\end{align}

\subsubsection{$\Vb_{4}$}
\begin{align}
\Delta&=((gp^2-2gnp+gn^2+(2d+2 e)l^2+(-2d-2 e)fg)q^2 +(c(-2mp^2+(4mn+(-2d-2 e)l)p-2mn^2+(-2d-2 e)ln +(4d+4 e)fm) +b((2d+2 e)gp+(2d+2 e)gn+(-4d-4 e)lm)) q +a((m^2-dg)p^2+((-2m^2-2 eg)n+(2d+2 e)lm)p +(m^2-dg)n^2+(2d+2 e)lmn +f((-2d-2 e)m^2+(d^2- e^2)g)+( e^2-d^2)l^2) +c^2(dp^2+2 enp+dn^2+( e^2-d^2)f) +bc((-2d-2 e)mp+(-2d-2 e)mn+(2d^2-2 e^2)l) +b^2((2d+2 e)m^2+( e^2-d^2)g))\nonumber
\end{align}

\begin{align}
A&=(2l^2-gh-fg)\nonumber\\
B&=\nonumber\\
C&=\nonumber\\
D&=\nonumber\\
E&=\nonumber\\
F&=\nonumber\\
G&=\nonumber\\
H&=\nonumber
\end{align}

\begin{align}
\alpha&=\frac{1}{\Delta}(-((gp^3+(-gn-2lm)p^2 +(-gn^2+4lmn+(d+ e)gh+(-d- e)fg)p+gn^3-2lmn^2\nonumber\\
& +((d+ e)gh+(-d- e)fg)n +l((-2d-2 e)hm+(2d+2 e)fm)) q \nonumber\\
&+c(-mp^3+(mn+(d- e)l)p^2 +(mn^2+(2 e-2d)ln+(-d- e)hm+(d+ e)fm)p\nonumber\\
&-mn^3 +(d- e)ln^2+((-d- e)hm+(d+ e)fm)n +((d^2- e^2)h+( e^2-d^2)f)l)\nonumber\\
& +b((2m^2+( e-d)g)p^2+((2d-2 e)g-4m^2)np +(2m^2+( e-d)g)n^2\nonumber\\
& +h((2d+2 e)m^2+( e^2-d^2)g) +f((-2d-2 e)m^2+(d^2- e^2)g))))\nonumber\\
\beta&=\frac{1}{\Delta}(((gp^2-2gnp+gn^2+(-2d-2 e)l^2+(2d+2 e)gh)q^2 \nonumber\\
&+(c(-2mp^2+(4mn+(2d+2 e)l)p-2mn^2+(2d+2 e)ln +(-4d-4 e)hm)\nonumber\\
& +b((-2d-2 e)gp+(-2d-2 e)gn+(4d+4 e)lm)) q +a((m^2+ eg)p^2\nonumber\\
&+((2dg-2m^2)n+(-2d-2 e)lm)p +(m^2+ eg)n^2+(-2d-2 e)lmn \nonumber\\
&+h((2d+2 e)m^2+( e^2-d^2)g)+(d^2- e^2)l^2) +c^2(- ep^2-2dnp- en^2+(d^2- e^2)h)\nonumber\\
& +bc((2d+2 e)mp+(2d+2 e)mn+(2 e^2-2d^2)l) +b^2((-2d-2 e)m^2+(d^2- e^2)g)))\nonumber\\
\gamma&=1\nonumber\\
\delta&=\frac{1}{\Delta}(-((2lp^2-4lnp+2ln^2+((2d+2 e)h+(-2d-2 e)f)l)q^2\nonumber\\
& +(c(-p^3+np^2+(n^2+(-d- e)h+(d+ e)f)p-n^3 +((-d- e)h+(d+ e)f)n)\nonumber\\
& +b(-2mp^2+4mnp-2mn^2+(-2d-2 e)hm+(2d+2 e)fm)) q +a(mp^3+(( e-d)l-mn)p^2\nonumber\\
& +(-mn^2+(2d-2 e)ln+(d+ e)hm+(-d- e)fm)p+mn^3 +( e-d)ln^2\nonumber\\
&+((d+ e)hm+(-d- e)fm)n +(( e^2-d^2)h+(d^2- e^2)f)l) +bc ((d- e)p^2\nonumber\\
&+(2 e-2d)np+(d- e)n^2+(d^2- e^2)h+( e^2-d^2)f)))\nonumber\\
\epsilon&=\frac{1}{\Delta}(-((Ap+(-2l^2+gh+fg)n)q^2\nonumber\\
& +(c(-3lp^2+(2ln+2hm+2fm)p+ln^2+(-2hm-2fm)n +((-d- e)h+(d+ e)f)l)\nonumber\\
& +b(3gp^2+(-2gn-4lm)p-gn^2+4lmn+(d+ e)gh+(-d- e)fg)) q \nonumber\\
&+a(-gp^3+3lmp^2 +(gn^2-2lmn+f(dg-m^2)+h(-m^2- eg)+( e-d)l^2)p\nonumber\\
& -lmn^2+(h(m^2-dg)+f(m^2+ eg)+(d- e)l^2)n +l((d+ e)hm+(-d- e)fm))\nonumber\\
& +c^2(p^3+(-n^2+ eh-df)p+(dh- ef)n) +bc (-3mp^2+(2mn+(2d-2 e)l)p+mn^2\nonumber\\
&+(2 e-2d)ln+(-d- e)hm +(d+ e)fm) +b^2((2m^2+( e-d)g)p+((d- e)g-2m^2)n)))\nonumber\\
\theta&=\frac{1}{\Delta}(-((Ap+(-2l^2+gh+fg)n)q^2\nonumber\\
& +(c(-lp^2+(-2ln+2hm+2fm)p+3ln^2+(-2hm-2fm)n +((d+ e)h+(-d- e)f)l)\nonumber\\
& +b(gp^2+(2gn-4lm)p-3gn^2+4lmn+(-d- e)gh+(d+ e)fg)) q \nonumber\\
&+a((lm-gn)p^2+(2lmn+h(dg-m^2)+f(-m^2- eg)+( e-d)l^2)p +gn^3\nonumber\\
&-3lmn^2 +(f(m^2-dg)+h(m^2+ eg)+(d- e)l^2)n +l((-d- e)hm+(d+ e)fm))\nonumber\\
& +c^2(np^2+( ef-dh)p-n^3+(df- eh)n) +bc (-mp^2+((2d-2 e)l-2mn)p+3mn^2\nonumber\\
&+(2 e-2d)ln+(d+ e)hm +(-d- e)fm)+b^2((2m^2+( e-d)g)p+((d- e)g-2m^2)n)))\nonumber
\end{align}

\subsubsection{$\Vb_{5}$}
\begin{align}
\Delta&=((gp^2-2gnp+gn^2+(2d+2 e)l^2+(-2d-2 e)fg)q^2 +(c(-2mp^2+(4mn+(-2d-2 e)l)p-2mn^2+(-2d-2 e)ln +(4d+4 e)fm) +b((2d+2 e)gp+(2d+2 e)gn+(-4d-4 e)lm)) q +a((m^2-dg)p^2+((-2m^2-2 eg)n+(2d+2 e)lm)p +(m^2-dg)n^2+(2d+2 e)lmn +f((-2d-2 e)m^2+(d^2- e^2)g)+( e^2-d^2)l^2) +c^2(dp^2+2 enp+dn^2+( e^2-d^2)f) +bc((-2d-2 e)mp+(-2d-2 e)mn+(2d^2-2 e^2)l) +b^2((2d+2 e)m^2+( e^2-d^2)g))\nonumber
\end{align}

\begin{align}
A&=(2l^2-gh-fg)\nonumber\\
B&=\nonumber\\
C&=\nonumber\\
D&=\nonumber\\
E&=\nonumber\\
F&=\nonumber\\
G&=\nonumber\\
H&=\nonumber
\end{align}
\begin{align}
\alpha &=\frac{ -((gp^3+(-gn-2lm)p^2 +(-gn^2+4lmn+(d+ e)gh+(-d- e)fg)p+gn^3-2lmn^2 +((d+ e)gh+(-d- e)fg)n +l((-2d-2 e)hm+(2d+2 e)fm)) q +c(-mp^3+(mn+(d- e)l)p^2 +(mn^2+(2 e-2d)ln+(-d- e)hm+(d+ e)fm)p-mn^3 +(d- e)ln^2+((-d- e)hm+(d+ e)fm)n +((d^2- e^2)h+( e^2-d^2)f)l) +b((2m^2+( e-d)g)p^2+((2d-2 e)g-4m^2)np +(2m^2+( e-d)g)n^2 +h((2d+2 e)m^2+( e^2-d^2)g) +f((-2d-2 e)m^2+(d^2- e^2)g))) }{\Delta}\nonumber\\ 
\beta&=1\nonumber\\
\gamma &=\frac{ ((gp^2-2gnp+gn^2+(-2d-2 e)l^2+(2d+2 e)gh)q^2 +(c(-2mp^2+(4mn+(2d+2 e)l)p-2mn^2+(2d+2 e)ln +(-4d-4 e)hm) +b((-2d-2 e)gp+(-2d-2 e)gn+(4d+4 e)lm)) q +a((m^2+ eg)p^2+((2dg-2m^2)n+(-2d-2 e)lm)p +(m^2+ eg)n^2+(-2d-2 e)lmn +h((2d+2 e)m^2+( e^2-d^2)g)+(d^2- e^2)l^2) +c^2(- ep^2-2dnp- en^2+(d^2- e^2)h) +bc((2d+2 e)mp+(2d+2 e)mn+(2 e^2-2d^2)l) +b^2((-2d-2 e)m^2+(d^2- e^2)g)) }{\Delta}\nonumber\\ 
\delta &= \frac{-((2lp^2-4lnp+2ln^2+((2d+2 e)h+(-2d-2 e)f)l)q^2 +(c(-p^3+np^2+(n^2+(-d- e)h+(d+ e)f)p-n^3 +((-d- e)h+(d+ e)f)n) +b(-2mp^2+4mnp-2mn^2+(-2d-2 e)hm+(2d+2 e)fm)) q +a(mp^3+(( e-d)l-mn)p^2 +(-mn^2+(2d-2 e)ln+(d+ e)hm+(-d- e)fm)p+mn^3 +( e-d)ln^2+((d+ e)hm+(-d- e)fm)n +(( e^2-d^2)h+(d^2- e^2)f)l) +bc ((d- e)p^2+(2 e-2d)np+(d- e)n^2+(d^2- e^2)h+( e^2-d^2)f)) }{\Delta}\nonumber\\ 
\epsilon &=\frac{ ((Ap+(-2l^2+gh+fg)n)q^2 +(c(-lp^2+(-2ln+2hm+2fm)p+3ln^2+(-2hm-2fm)n +((d+ e)h+(-d- e)f)l) +b(gp^2+(2gn-4lm)p-3gn^2+4lmn+(-d- e)gh+(d+ e)fg)) q +a((lm-gn)p^2+(2lmn+h(dg-m^2)+f(-m^2- eg)+( e-d)l^2)p +gn^3-3lmn^2 +(f(m^2-dg)+h(m^2+ eg)+(d- e)l^2)n +l((-d- e)hm+(d+ e)fm)) +c^2(np^2+( ef-dh)p-n^3+(df- eh)n) +bc (-mp^2+((2d-2 e)l-2mn)p+3mn^2+(2 e-2d)ln+(d+ e)hm +(-d- e)fm)+b^2((2m^2+( e-d)g)p+((d- e)g-2m^2)n)) }{\Delta}\nonumber\\ 
\theta &=\frac{ ((Ap+(-2l^2+gh+fg)n)q^2 +(c(-3lp^2+(2ln+2hm+2fm)p+ln^2+(-2hm-2fm)n +((-d- e)h+(d+ e)f)l) +b(3gp^2+(-2gn-4lm)p-gn^2+4lmn+(d+ e)gh+(-d- e)fg)) q +a(-gp^3+3lmp^2 +(gn^2-2lmn+f(dg-m^2)+h(-m^2- eg)+( e-d)l^2)p -lmn^2+(h(m^2-dg)+f(m^2+ eg)+(d- e)l^2)n +l((d+ e)hm+(-d- e)fm)) +c^2(p^3+(-n^2+ eh-df)p+(dh- ef)n) +bc (-3mp^2+(2mn+(2d-2 e)l)p+mn^2+(2 e-2d)ln+(-d- e)hm +(d+ e)fm) +b^2((2m^2+( e-d)g)p+((d- e)g-2m^2)n)) }{\Delta}\nonumber
\end{align}

\subsubsection{$\Vb_{6}$}
\begin{align}
\Delta&=g(p+n)^2+(h+f)(2m^2+( e-d)g)+2(d-e)l^2-4lm(n+p)\,,\nonumber
\end{align}

\begin{align}
\alpha&=1\nonumber\\
\beta&=\gamma=\frac{l(2mq+c( e-d))+(p+n)(cm-gq)+b((d- e)g-2m^{2})}{\Delta}\nonumber\\
\delta& =-\frac{(f+h)(2mq+c( e-d))-2(p+n)(lq+bm)+c(p+n)^2+2bl(d-e)}{\Delta}\nonumber\\
\epsilon&=-\theta=\frac{(h+f)(gq-cm)+(cl-bg)(p+n)+2l(bm-lq)}{\Delta}\nonumber
\end{align}


\subsection{The eigenvectors in the subspace $\caM_{2}$}

\subsubsection{$\Vb_{1}$}

\begin{align}
\Delta&=\nonumber\\
\end{align}

\begin{align}
\alpha&=\frac{ ( ehn^3+(-2ghm+c(2h^2+ ef)- edg)n^2 +(fhm^2+(d(2g^2-2h^2)-2cfg)m +a(h^3+(g^2- ef)h)+b(-gh^2-g^3+ efg) -4cdgh+3c^2fh+ ed^2h) n+(cf^2-dfg)m^2 +(b(fh^2+fg^2- ef^2)+2d^2gh-2cdfh)m +d(b(( ef-g^2)h-h^3)+a(-gh^2-g^3+ efg)-3c^2fg) +ac(fh^2+fg^2- ef^2)+cd^2(2g^2+ ef)- ed^3g +c^3f^2) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)-2bgh-2cdg+c^2f +2 ed^2) n^2 +((2bfh+2afg-2d^2g)m+bd(2g^2-2h^2) +c(-2afh-2bfg) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh-2bfg)-2d^3h+2bcf^2)m +d^2(a(h^2+g^2-2 ef)+2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2afg-2bfh)-2cd^3g-ac^2f^2+ ed^4)}\nonumber\\ 
\beta&=\frac{ ( egn^3+((-2g^2- ef)m+2cgh+ edh)n^2 +(3fgm^2+(-4dgh-2cfh)m+b(( ef-g^2)h-h^3) +a(gh^2+g^3- efg)+cd(2h^2-2g^2) +c^2fg+ ed^2g) n-f^2m^3+3dfhm^2 +(a(-fh^2-fg^2+ ef^2)+d^2(-2h^2- ef)+2cdfg -c^2f^2) m+d(a(h^3+(g^2- ef)h)+b(gh^2+g^3- efg)+c^2fh) +bc(-fh^2-fg^2+ ef^2)-2cd^2gh+ ed^3h) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)-2bgh-2cdg+c^2f +2 ed^2) n^2 +((2bfh+2afg-2d^2g)m+bd(2g^2-2h^2) +c(-2afh-2bfg) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh-2bfg)-2d^3h+2bcf^2)m +d^2(a(h^2+g^2-2 ef)+2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2afg-2bfh)-2cd^3g-ac^2f^2+ ed^4)}\nonumber\\ 
\gamma&=\frac{ -(b(h^2-g^2)n^2+(2bfgm-4bdgh+2bcfh)n-bf^2m^2 +2bdfhm+bd^2(g^2-h^2)-2bcdfg +bc^2f^2) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)-2bgh-2cdg+c^2f +2 ed^2) n^2 +((2bfh+2afg-2d^2g)m+bd(2g^2-2h^2) +c(-2afh-2bfg) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh-2bfg)-2d^3h+2bcf^2)m +d^2(a(h^2+g^2-2 ef)+2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2afg-2bfh)-2cd^3g-ac^2f^2+ ed^4)}\nonumber\\ 
\delta&=\frac{ -( emn^3+(-2gm^2+2chm- ebh- eag+ ecd)n^2 +(fm^3-2dhm^2 +(a(h^2+3g^2- ef)-4cdg+c^2f+ ed^2)m +c(b(-h^2-g^2- ef)-2agh) +d(2c^2h+2 ebg)) n+(bfh-afg+cdf)m^2 +(d(b(-h^2-g^2- ef)+2agh)-2cd^2h+2bcfg)m +d(ac(h^2+3g^2- ef)+c^3f)+b^2(gh^2+g^3- efg) +a^2(-gh^2-g^3+ efg)+c^2(-bfh-afg) +d^2( ebh-2c^2g- eag)+ ecd^3) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)-2bgh-2cdg+c^2f +2 ed^2) n^2 +((2bfh+2afg-2d^2g)m+bd(2g^2-2h^2) +c(-2afh-2bfg) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh-2bfg)-2d^3h+2bcf^2)m +d^2(a(h^2+g^2-2 ef)+2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2afg-2bfh)-2cd^3g-ac^2f^2+ ed^4)}\nonumber\\ 
\epsilon&=\frac{ -( ecn^3+((-2cg- ed)m+2c^2h+ eah+ ebg)n^2 +((2dg+cf)m^2+(b(-h^2-g^2- ef)-2agh-4cdh)m +ac(3h^2+g^2- ef) +d(2 ebh-2c^2g)+c^3f+ ecd^2) n-dfm^3+(afh+2d^2h+bfg)m^2 +(d(a(-3h^2-g^2+ ef)-c^2f) -2bcfh+2cd^2g- ed^3) m+a^2(h^3+(g^2- ef)h)+b^2(( ef-g^2)h-h^3) +cd(b(h^2+g^2+ ef)-2agh)+c^2(afh-bfg) +d^2( eah- ebg)) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)-2bgh-2cdg+c^2f +2 ed^2) n^2 +((2bfh+2afg-2d^2g)m+bd(2g^2-2h^2) +c(-2afh-2bfg) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh-2bfg)-2d^3h+2bcf^2)m +d^2(a(h^2+g^2-2 ef)+2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2afg-2bfh)-2cd^3g-ac^2f^2+ ed^4)}\nonumber\\
\theta&=1\nonumber
\end{align}

\subsubsection{$Vb_{2}$}

\begin{align}
\Delta&=\nonumber\\
\end{align}

\begin{align}
\alpha&=\frac{ ( e^2n^3+( ech-3 egm)n^2 +((-2h^2+2g^2+ ef)m^2-2cghm +a( eh^2+ eg^2- e^2f) +c^2( ef-2h^2)-2 ebgh -2 ecdg+ e^2d^2) n-fgm^3+(2dgh-cfh)m^2 +(b((g^2+ ef)h-h^3)+a(gh^2-g^3+ efg)+2cdg^2 -c^2fg- ed^2g) m+c(a((g^2+ ef)h-h^3)+b(-gh^2+g^3- efg)) +d(b(- eh^2- eg^2+ e^2f)-2 eagh)-c^3fh + ecd^2h) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(2 ebh-2c^2g+2 eag)m +c(2 ebg-2 eah)+2c^3h -2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)-2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2h^2-2g^2) +d(-2c^2h+2 eah+2 ebg)) m+c^2(a(h^2+g^2-2 ef)+2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 eag-2 ebh)-2c^3g)+c^4f +( ec^2- e^2a)d^2)}\nonumber\\ 
\beta&=\frac{ -(( ehm+ ecg- e^2d)n^2 +((2 edg-2cg^2)m+b( eh^2+ eg^2- e^2f)+2c^2gh -2 eagh) n-fhm^3+(d(2h^2- ef)+cfg)m^2 +(a((g^2+ ef)h-h^3)+b(gh^2-g^3+ efg)-2cdgh-c^2fh + ed^2h) m+c(b((g^2+ ef)h-h^3)+a(-gh^2+g^3- efg)) +d(a(- eh^2- eg^2+ e^2f)+c^2(2h^2-2g^2- ef)-2 ebgh) +c^3fg+3 ecd^2g- e^2d^3) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(2 ebh-2c^2g+2 eag)m +c(2 ebg-2 eah)+2c^3h -2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)-2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2h^2-2g^2) +d(-2c^2h+2 eah+2 ebg)) m+c^2(a(h^2+g^2-2 ef)+2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 eag-2 ebh)-2c^3g)+c^4f +( ec^2- e^2a)d^2)}\nonumber\\ 
\gamma&=\frac{ -( emn^3+(-2gm^2+ ebh- eag+ ecd)n^2 +(fm^3+(a(-h^2+3g^2- ef)-2bgh-4cdg+c^2f + ed^2) m+bc(-h^2+g^2+ ef)-2 ebdg) n+(bfh-afg+cdf)m^2 +(bd(-h^2+g^2+ ef)-2bcfg)m +a^2(gh^2-g^3+ efg)+b^2(-gh^2+g^3- efg) +d(c(a(-h^2+3g^2- ef)+2bgh)+c^3f) +c^2(-bfh-afg)+d^2(- ebh-2c^2g- eag) + ecd^3) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(2 ebh-2c^2g+2 eag)m +c(2 ebg-2 eah)+2c^3h -2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)-2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2h^2-2g^2) +d(-2c^2h+2 eah+2 ebg)) m+c^2(a(h^2+g^2-2 ef)+2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 eag-2 ebh)-2c^3g)+c^4f +( ec^2- e^2a)d^2)}\nonumber\\ 
\delta&=\frac{ ( e^2bn^2+(2hm^3+(2c^2h-2 eah-2 ebg)m)n +(b(h^2+g^2)-2agh+2cdh)m^2 +c^2(b(-h^2-g^2)-2agh) +d(c(2 ebg-2 eah)+2c^3h)-2 eb^2gh +2 ea^2gh- e^2bd^2) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(2 ebh-2c^2g+2 eag)m +c(2 ebg-2 eah)+2c^3h -2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)-2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2h^2-2g^2) +d(-2c^2h+2 eah+2 ebg)) m+c^2(a(h^2+g^2-2 ef)+2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 eag-2 ebh)-2c^3g)+c^4f +( ec^2- e^2a)d^2)}\nonumber\\ 
\epsilon&=1\nonumber\\
\theta&=\frac{ -( ecn^3+(2hm^2+(-2cg- ed)m+2c^2h- eah+ ebg)n^2 +((2dg+cf)m^2+(b(3h^2-g^2- ef)-2agh)m +ac(-h^2+g^2- ef) +d(-2 ebh-2c^2g)+c^3f+ ecd^2) n-dfm^3+(-afh+2d^2h+bfg)m^2 +(d(a(h^2-g^2+ ef)-c^2f)+2bcfh+2cd^2g- ed^3) m+b^2(h^3+(-g^2- ef)h)+a^2((g^2+ ef)h-h^3) +cd(b(-3h^2+g^2+ ef)-2agh)+c^2(-afh-bfg) +d^2(2c^2h- eah- ebg)) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(2 ebh-2c^2g+2 eag)m +c(2 ebg-2 eah)+2c^3h -2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)-2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2h^2-2g^2) +d(-2c^2h+2 eah+2 ebg)) m+c^2(a(h^2+g^2-2 ef)+2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 eag-2 ebh)-2c^3g)+c^4f +( ec^2- e^2a)d^2)}\nonumber
\end{align}

\subsubsection{$Vb_{3}$}

\begin{align}
\Delta&=\nonumber\\
\end{align}

\begin{align}
\alpha&=\frac{ -(( ehm+ ecg- e^2d)n^2 +(-2ghm^2+(c(2h^2-2g^2)+2 edg)m+b(- eh^2- eg^2+ e^2f) +2c^2gh-2 ecdh) n+fhm^3+(d(-2h^2- ef)+cfg)m^2 +(a(h^3+(g^2- ef)h)+b(gh^2+g^3- efg)-4cdgh+c^2fh +3 ed^2h) m+c(b(( ef-g^2)h-h^3)+a(gh^2+g^3- efg)) +d(a(- eh^2- eg^2+ e^2f)+c^2(-2g^2- ef))+c^3fg +3 ecd^2g- e^2d^3) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(-2 ebh-2c^2g+2 eag) m+c(-2 eah-2 ebg) +2c^3h+2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)+2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2g^2-2h^2) +d(-2c^2h+2 eah-2 ebg)) m+c^2(a(h^2+g^2-2 ef)-2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 ebh+2 eag)-2c^3g)+c^4f +( ec^2- e^2a)d^2)} 
\beta&=\frac{ -( e^2n^3+(3 ech-3 egm)n^2 +((2g^2+ ef)m^2+(-4cgh-2 edh)m +a( eh^2+ eg^2- e^2f) +c^2(2h^2+ ef)-2 ecdg+ e^2d^2) n-fgm^3+(2dgh+cfh)m^2 +(b(( ef-g^2)h-h^3)+a(-gh^2-g^3+ efg) +cd(2g^2-2h^2)-c^2fg - ed^2g) m+c(a(h^3+(g^2- ef)h)+b(-gh^2-g^3+ efg)) +d(b( eh^2+ eg^2- e^2f)-2c^2gh)+c^3fh + ecd^2h) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(-2 ebh-2c^2g+2 eag) m+c(-2 eah-2 ebg) +2c^3h+2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)+2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2g^2-2h^2) +d(-2c^2h+2 eah-2 ebg)) m+c^2(a(h^2+g^2-2 ef)-2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 ebh+2 eag)-2c^3g)+c^4f +( ec^2- e^2a)d^2)} 
\gamma&=\frac{ ( ecn^3+((-2cg- ed)m+2c^2h+ eah- ebg)n^2 +((2dg+cf)m^2+(b(h^2+g^2+ ef)-2agh-4cdh)m +ac(3h^2+g^2- ef) +d(-2 ebh-2c^2g)+c^3f+ ecd^2) n-dfm^3+(afh+2d^2h-bfg)m^2 +(d(a(-3h^2-g^2+ ef)-c^2f) +2bcfh+2cd^2g- ed^3) m+a^2(h^3+(g^2- ef)h)+b^2(( ef-g^2)h-h^3) +cd(b(-h^2-g^2- ef)-2agh)+c^2(afh+bfg) +d^2( eah+ ebg)) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(-2 ebh-2c^2g+2 eag) m+c(-2 eah-2 ebg) +2c^3h+2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)+2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2g^2-2h^2) +d(-2c^2h+2 eah-2 ebg)) m+c^2(a(h^2+g^2-2 ef)-2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 ebh+2 eag)-2c^3g)+c^4f +( ec^2- e^2a)d^2)} 
\delta&=1\nonumber\\
\epsilon&=\frac{ ( e^2bn^2+(2 ebch-2 ebgm)n+b(g^2-h^2)m^2 +(2 ebdh-4bcgh)m+bc^2(h^2-g^2)+2 ebcdg - e^2bd^2) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(-2 ebh-2c^2g+2 eag) m+c(-2 eah-2 ebg) +2c^3h+2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)+2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2g^2-2h^2) +d(-2c^2h+2 eah-2 ebg)) m+c^2(a(h^2+g^2-2 ef)-2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 ebh+2 eag)-2c^3g)+c^4f +( ec^2- e^2a)d^2)} 
\theta&=\frac{ -( emn^3+(-2gm^2+2chm- ebh- eag+ ecd)n^2 +(fm^3-2dhm^2 +(a(h^2+3g^2- ef)-4cdg+c^2f+ ed^2)m +c(b(-h^2-g^2- ef)-2agh) +d(2c^2h+2 ebg)) n+(bfh-afg+cdf)m^2 +(d(b(-h^2-g^2- ef)+2agh)-2cd^2h+2bcfg)m +d(ac(h^2+3g^2- ef)+c^3f)+b^2(gh^2+g^3- efg) +a^2(-gh^2-g^3+ efg)+c^2(-bfh-afg) +d^2( ebh-2c^2g- eag)+ ecd^3) }{(( em^2+ ec^2- e^2a)n^2+(-2gm^3+2chm^2 +(-2 ebh-2c^2g+2 eag) m+c(-2 eah-2 ebg) +2c^3h+2 e^2bd) n+fm^4-2dhm^3 +(a(h^2+g^2-2 ef)+2bgh-2cdg +2c^2f+ ed^2) m^2 +(bc(2g^2-2h^2) +d(-2c^2h+2 eah-2 ebg)) m+c^2(a(h^2+g^2-2 ef)-2bgh) +b^2( eh^2+ eg^2- e^2f) +a^2(- eh^2- eg^2+ e^2f) +d(c(2 ebh+2 eag)-2c^3g)+c^4f +( ec^2- e^2a)d^2)}\nonumber
\end{align}

\subsubsection{$Vb_{4}$}

\begin{align}
\Delta&=\nonumber\\
\end{align}

\begin{align}
\alpha&=\frac{ -( egn^3+((-2g^2- ef)m+2cgh+ edh)n^2 +(3fgm^2+(-4dgh-2cfh)m+b(h^3+(g^2- ef)h) +a(gh^2+g^3- efg)+cd(2h^2-2g^2) +c^2fg+ ed^2g) n-f^2m^3+3dfhm^2 +(a(-fh^2-fg^2+ ef^2)+d^2(-2h^2- ef)+2cdfg -c^2f^2) m +d(a(h^3+(g^2- ef)h)+b(-gh^2-g^3+ efg)+c^2fh) +bc(fh^2+fg^2- ef^2)-2cd^2gh+ ed^3h) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)+2bgh-2cdg+c^2f +2 ed^2) n^2 +((-2bfh+2afg-2d^2g)m+bd(2h^2-2g^2) +c(2bfg-2afh) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh+2bfg)-2d^3h-2bcf^2)m +d^2(a(h^2+g^2-2 ef)-2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2bfh+2afg)-2cd^3g-ac^2f^2+ ed^4)} \nonumber\\
\beta&=\frac{ ( ehn^3+(-2ghm+c(2h^2+ ef)- edg)n^2 +(fhm^2+(d(2g^2-2h^2)-2cfg)m +a(h^3+(g^2- ef)h)+b(gh^2+g^3- efg) -4cdgh+3c^2fh+ ed^2h) n+(cf^2-dfg)m^2 +(b(-fh^2-fg^2+ ef^2)+2d^2gh-2cdfh)m +d(b(h^3+(g^2- ef)h)+a(-gh^2-g^3+ efg)-3c^2fg) +ac(fh^2+fg^2- ef^2)+cd^2(2g^2+ ef)- ed^3g +c^3f^2) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)+2bgh-2cdg+c^2f +2 ed^2) n^2 +((-2bfh+2afg-2d^2g)m+bd(2h^2-2g^2) +c(2bfg-2afh) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh+2bfg)-2d^3h-2bcf^2)m +d^2(a(h^2+g^2-2 ef)-2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2bfh+2afg)-2cd^3g-ac^2f^2+ ed^4)} \nonumber\\
\gamma&=1\nonumber\\
\delta&=\frac{ ( ecn^3+((-2cg- ed)m+2c^2h+ eah- ebg)n^2 +((2dg+cf)m^2+(b(h^2+g^2+ ef)-2agh-4cdh)m +ac(3h^2+g^2- ef) +d(-2 ebh-2c^2g)+c^3f+ ecd^2) n-dfm^3+(afh+2d^2h-bfg)m^2 +(d(a(-3h^2-g^2+ ef)-c^2f) +2bcfh+2cd^2g- ed^3) m+a^2(h^3+(g^2- ef)h)+b^2(( ef-g^2)h-h^3) +cd(b(-h^2-g^2- ef)-2agh)+c^2(afh+bfg) +d^2( eah+ ebg)) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)+2bgh-2cdg+c^2f +2 ed^2) n^2 +((-2bfh+2afg-2d^2g)m+bd(2h^2-2g^2) +c(2bfg-2afh) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh+2bfg)-2d^3h-2bcf^2)m +d^2(a(h^2+g^2-2 ef)-2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2bfh+2afg)-2cd^3g-ac^2f^2+ ed^4)} \nonumber\\
\epsilon&=\frac{ -( emn^3+(-2gm^2+2chm+ ebh- eag+ ecd)n^2 +(fm^3-2dhm^2 +(a(h^2+3g^2- ef)-4cdg+c^2f+ ed^2)m +c(b(h^2+g^2+ ef)-2agh) +d(2c^2h-2 ebg)) n+(-bfh-afg+cdf)m^2 +(d(b(h^2+g^2+ ef)+2agh)-2cd^2h-2bcfg)m +d(ac(h^2+3g^2- ef)+c^3f)+b^2(gh^2+g^3- efg) +a^2(-gh^2-g^3+ efg)+c^2(bfh-afg) +d^2(- ebh-2c^2g- eag)+ ecd^3) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)+2bgh-2cdg+c^2f +2 ed^2) n^2 +((-2bfh+2afg-2d^2g)m+bd(2h^2-2g^2) +c(2bfg-2afh) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh+2bfg)-2d^3h-2bcf^2)m +d^2(a(h^2+g^2-2 ef)-2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2bfh+2afg)-2cd^3g-ac^2f^2+ ed^4)} \nonumber\\
\theta&=\frac{ -(b(h^2-g^2)n^2+(2bfgm-4bdgh+2bcfh)n-bf^2m^2 +2bdfhm+bd^2(g^2-h^2)-2bcdfg +bc^2f^2) }{( en^4+(2ch-2gm)n^3 +(fm^2-2dhm+a(h^2+g^2-2 ef)+2bgh-2cdg+c^2f +2 ed^2) n^2 +((-2bfh+2afg-2d^2g)m+bd(2h^2-2g^2) +c(2bfg-2afh) +2cd^2h) n+(d^2f-af^2)m^2 +(d(2afh+2bfg)-2d^3h-2bcf^2)m +d^2(a(h^2+g^2-2 ef)-2bgh+c^2f) +b^2(fh^2+fg^2- ef^2)+a^2(-fh^2-fg^2+ ef^2) +cd(2bfh+2afg)-2cd^3g-ac^2f^2+ ed^4)}\nonumber
\end{align}

\subsubsection{$\Vb_{5}$}

\begin{align}
\Delta&=\nonumber\\
\end{align}

\begin{align}
\alpha&=\frac{ ((cgh- egh)n^2+(( efh-cfh)m +d(c(h^2-g^2)- eh^2+ eg^2)+c^2fg - ecfg) n+(d(cfg- efg)-c^2f^2+ ecf^2)m +b(-h^4+( ef-2g^2)h^2-g^4+ efg^2) +bc(fh^2+fg^2- ef^2)+d^2( egh-cgh) +d(c^2fh- ecfh)) }{(( eh^2+c(g^2- ef))n^2+((-2gh^2-2g^3+2 efg)m +c(2h^3+2g^2h)+d(2cgh-2 egh) -2c^2fh) n+(fh^2+fg^2- ef^2)m^2 +d((2 ef-2g^2)h-2h^3)m +a(h^4+(2g^2- ef)h^2+g^4- efg^2) +d(c(-2gh^2-2g^3)+2c^2fg) +d^2(c(h^2- ef)+ eg^2) +c^2(fh^2+fg^2) +ac(-fh^2-fg^2+ ef^2)-c^3f^2)}\nonumber\\ 
\beta&=1\nonumber\\
\gamma&=\frac{ ( ehn^3+(-2ghm+c(2h^2+ ef)- edg)n^2 +(fhm^2+(d(2g^2-2h^2)-2cfg)m +a(h^3+(g^2- ef)h)+b(gh^2+g^3- efg) -4cdgh+3c^2fh+ ed^2h) n+(cf^2-dfg)m^2 +(b(-fh^2-fg^2+ ef^2)+2d^2gh-2cdfh)m +d(b(h^3+(g^2- ef)h)+a(-gh^2-g^3+ efg)-3c^2fg) +ac(fh^2+fg^2- ef^2)+cd^2(2g^2+ ef)- ed^3g +c^3f^2) }{(( eh^2+c(g^2- ef))n^2+((-2gh^2-2g^3+2 efg)m +c(2h^3+2g^2h)+d(2cgh-2 egh) -2c^2fh) n+(fh^2+fg^2- ef^2)m^2 +d((2 ef-2g^2)h-2h^3)m +a(h^4+(2g^2- ef)h^2+g^4- efg^2) +d(c(-2gh^2-2g^3)+2c^2fg) +d^2(c(h^2- ef)+ eg^2) +c^2(fh^2+fg^2) +ac(-fh^2-fg^2+ ef^2)-c^3f^2)}\nonumber\\ 
\delta&=\frac{ -( ecn^3+((-cg-2 eg)m+2c^2h+ ech)n^2 +((2g^2+ ef)m^2+(d(-ch- eh)-4cgh)m +c(a(h^2- ef)+bgh)+2c^2h^2 - ebgh+ eag^2+d(-c^2g- ecg) +c^3f+ ecd^2) n-fgm^3+(2dgh+cfh)m^2 +(b(( ef-g^2)h-h^3)+a(-gh^2-g^3) +d(c(-2h^2+2g^2+ ef)-c^2f) -c^2fg+acfg- ed^2g) m+c(a(h^3+(g^2- ef)h)+b(-gh^2-g^3)) +d(c(b(h^2- ef)-agh)-2c^2gh+ eagh+ ebg^2) +c^3fh+c^2d^2h+bc^2fg) }{(( eh^2+c(g^2- ef))n^2+((-2gh^2-2g^3+2 efg)m +c(2h^3+2g^2h)+d(2cgh-2 egh) -2c^2fh) n+(fh^2+fg^2- ef^2)m^2 +d((2 ef-2g^2)h-2h^3)m +a(h^4+(2g^2- ef)h^2+g^4- efg^2) +d(c(-2gh^2-2g^3)+2c^2fg) +d^2(c(h^2- ef)+ eg^2) +c^2(fh^2+fg^2) +ac(-fh^2-fg^2+ ef^2)-c^3f^2)}\nonumber\\ 
\epsilon&=\frac{ -(( ehm+c^2g- ecd)n^2+(-2ghm^2 +(c(2h^2-2g^2+ ef) +d(cg+ eg)-c^2f) m+ ebh^2+c(agh+b(g^2- ef)) +d(-c^2h- ech)+2c^2gh- eagh) n+fhm^3+(d(-2h^2- ef)+cfg)m^2 +(a(h^3+g^2h)+b(-gh^2-g^3+ efg) +d^2(ch+2 eh) -4cdgh+c^2fh -acfh) m +c(b(h^3+g^2h)+a(gh^2+g^3- efg)) +d (- eah^2+c(bgh+a( ef-g^2)) - ebgh-2c^2g^2-c^3f) -bc^2fh+d^2(2c^2g+ ecg)+c^3fg - ecd^3) }{(( eh^2+c(g^2- ef))n^2+((-2gh^2-2g^3+2 efg)m +c(2h^3+2g^2h)+d(2cgh-2 egh) -2c^2fh) n+(fh^2+fg^2- ef^2)m^2 +d((2 ef-2g^2)h-2h^3)m +a(h^4+(2g^2- ef)h^2+g^4- efg^2) +d(c(-2gh^2-2g^3)+2c^2fg) +d^2(c(h^2- ef)+ eg^2) +c^2(fh^2+fg^2) +ac(-fh^2-fg^2+ ef^2)-c^3f^2)}\nonumber\\ 
\theta&=\frac{ (cgn^3+((-2g^2-cf)m+2cgh+cdh)n^2 +(3fgm^2+(-4dgh-2cfh)m+b(-h^3-g^2h) +a(gh^2+g^3)+cd(2h^2-2g^2) +c(bfh-afg)+c^2fg+cd^2g) n-f^2m^3+3dfhm^2 +(a(-fh^2-fg^2)+d^2(-2h^2-cf)+2cdfg-c^2f^2 +acf^2) m +d(a(h^3+g^2h)+b(gh^2+g^3)+c(-afh-bfg)+c^2fh) +bc(-fh^2-fg^2)-2cd^2gh+cd^3h+bc^2f^2) }{(( eh^2+c(g^2- ef))n^2+((-2gh^2-2g^3+2 efg)m +c(2h^3+2g^2h)+d(2cgh-2 egh) -2c^2fh) n+(fh^2+fg^2- ef^2)m^2 +d((2 ef-2g^2)h-2h^3)m +a(h^4+(2g^2- ef)h^2+g^4- efg^2) +d(c(-2gh^2-2g^3)+2c^2fg) +d^2(c(h^2- ef)+ eg^2) +c^2(fh^2+fg^2) +ac(-fh^2-fg^2+ ef^2)-c^3f^2)}\nonumber
\end{align}

\subsection{$\Vb_{6}$}

\begin{align}
\Delta&=\nonumber\\
\end{align}

\begin{align}
\alpha&=1\nonumber\\
\beta&=\frac{ -(((h+ e)m-bh- ed)n-gm^2+c(h+f)m+a(-h^2-g^2+ ef) +d(bg-ch)-bcf) }{((gm-ch- eh)n-fm^2+(gh+2dh)m-ch^2+a(-h^2-g^2+ ef) +2cdg-c^2f- ed^2)}\nonumber\\ 
\gamma &=\frac{ -((g^2m-cgh- egh)n^2+((gh-fg)m^2 +(h^3+c(-h^2+fh+ ef)+d(gh- eg) +g^2h-bfg) m-bh^3+a(-gh^2-g^3+ efg) +d(- eh^2+bgh+c(2g^2- ef)) -cgh^2+ ebfh-c^2fg) n-fhm^3 +(d(2h^2+g^2)-cfg+bf^2)m^2 +(a(( ef-g^2)h-h^3) +cfh^2+d(c(gh-fg)-2bfh) -bfgh- ed^2h+c^2f^2) m +a (-h^4+(-g^2+bf+ ef)h^2+bfg^2 - ebf^2) +d (-ch^3+a(gh^2+g^3- efg)+bgh^2 -c^2fh) +ac(-fh^2-fg^2+ ef^2) +d^2(cgh-bg^2+ ebf)) }{(((gh^2+g^3- efg)m- eh^3+c(( ef-g^2)h-h^3) +( e^2f- eg^2)h) n +(-fh^2-fg^2+ ef^2)m^2 +(d(2h^3+(2g^2-2 ef)h)+gh^3+(g^3- efg)h)m +c(( ef-g^2)h^2-h^4) +a(-h^4+(2 ef-2g^2)h^2-g^4+2 efg^2- e^2f^2) +cd(2gh^2+2g^3-2 efg)+c^2(-fh^2-fg^2+ ef^2) +d^2(- eh^2- eg^2+ e^2f))}\nonumber\\ 
\delta &=\frac{ -((ghm^2+(- eh^2+c(g^2-h^2)- edg)m+d( ech+ e^2h) -c^2gh- ecgh) n +( ef-g^2)m^3+(2cgh-bfh-2 edh)m^2 +(a(( e-g)h^2-g^3+ eg^2+ efg- e^2f) +d(2bh^2+c(gh-2 eg)+bg^2)+bgh^2+c^2(-h^2-fh+ ef) +c((g^2- ef)h-bfg)+ e^2d^2) m+c(a(h^3-gh^2+(g^2- ef)h-g^3+ efg)-bh^3+ ebfh) +a(( e-b)h^3+(( e-b)g^2+ ebf- e^2f)h) +d(c( eh^2+bgh)+c^2(h^2+2g^2)- ebgh)-c^2gh^2 +d^2(- ebh- ecg)-c^3fg) }{(((gh^2+g^3- efg)m- eh^3+c(( ef-g^2)h-h^3) +( e^2f- eg^2)h) n +(-fh^2-fg^2+ ef^2)m^2 +(d(2h^3+(2g^2-2 ef)h)+gh^3+(g^3- efg)h)m +c(( ef-g^2)h^2-h^4) +a(-h^4+(2 ef-2g^2)h^2-g^4+2 efg^2- e^2f^2) +cd(2gh^2+2g^3-2 efg)+c^2(-fh^2-fg^2+ ef^2) +d^2(- eh^2- eg^2+ e^2f))}\nonumber\\ 
\epsilon&=\frac{ (( egm- ech- e^2h)n^2+((h^2+ eh- ef)m^2 +(-bh^2+c(2gh+ eg)+ egh-bg^2 - e^2d) m+a(- eh^2- eg^2+ e^2f) -2 ech^2+c^2(-h^2- ef) +d( ebh+ ecg)+ ebgh) n-ghm^3 +(c(h^2-g^2)+bfg+ edg)m^2 +(a(( ef-g^2)h-h^3) +d(c(h^2- eh- ef)-bgh) +c(gh^2-bfh)+c^2(gh+fg) -bg^2h) m-c^2h^3 +c (a (-h^3-gh^2+( ef-g^2)h-g^3+ efg) +bgh^2) +d (a( eh^2+ eg^2- e^2f) +c^2gh+c( ebf-bg^2)) +a(bgh^2+bg^3- ebfg)-c^3fh) }{(((gh^2+g^3- efg)m- eh^3+c(( ef-g^2)h-h^3) +( e^2f- eg^2)h) n +(-fh^2-fg^2+ ef^2)m^2 +(d(2h^3+(2g^2-2 ef)h)+gh^3+(g^3- efg)h)m +c(( ef-g^2)h^2-h^4) +a(-h^4+(2 ef-2g^2)h^2-g^4+2 efg^2- e^2f^2) +cd(2gh^2+2g^3-2 efg)+c^2(-fh^2-fg^2+ ef^2) +d^2(- eh^2- eg^2+ e^2f))}\nonumber\\ 
\theta &=\frac{ ((ghm-ch^2- eh^2)n^2+(( ef-g^2)m^2 +(d(h^2- eh- ef)+c(gh+fg)-bfh)m +a(( ef-g^2)h-h^3)+c(-h^3- efh) +d(bh^2+2cgh+ egh)+bgh^2 -2c^2fh) n+(cfh-dgh)m^2 +(a((g-f)h^2+g^3-fg^2- efg+ ef^2) +d(c(-h^2-2g^2)+bfg)+c^2fg + ed^2g-bcf^2) m +d(a(h^3+(g^2- ef)h) +c(gh^2+bfh)-bg^2h+2c^2fg) +a(gh^3+(g^3- efg)h) +c(a(-fh^2-fg^2+ ef^2)+bfgh) +d^2(c(h^2- ef)-bgh)-c^2fh^2 -c^3f^2) }{(((gh^2+g^3- efg)m- eh^3+c(( ef-g^2)h-h^3) +( e^2f- eg^2)h) n +(-fh^2-fg^2+ ef^2)m^2 +(d(2h^3+(2g^2-2 ef)h)+gh^3+(g^3- efg)h)m +c(( ef-g^2)h^2-h^4) +a(-h^4+(2 ef-2g^2)h^2-g^4+2 efg^2- e^2f^2) +cd(2gh^2+2g^3-2 efg)+c^2(-fh^2-fg^2+ ef^2) +d^2(- eh^2- eg^2+ e^2f))}\nonumber
\end{align}

\begin{align}
\lambda_1&= a-c \nonumber\\ 
\lambda_2&= \frac{1}{2} \left(-\sqrt{a^2-2 a b+2 a c+b^2-2 b c+c^2+8 d^2}+a+b+c\right) \nonumber\\ 
\lambda_3&= \frac{1}{2} \left(\sqrt{a^2-2 a b+2 a c+b^2-2 b c+c^2+8 d^2}+a+b+c\right) \nonumber\\ 
{v_1}&= \{-1,1,0\} \nonumber\\ 
{v_2}&= \left\{\frac{d^2-c\left(-\lambda_{2}+b\right)}{-d(c+\lambda_{2})}-\frac{-\lambda_{2}+b}{d},-\frac{d^2-c \left(-\lambda_{2}+b\right)}{-d(\lambda_{2}+c)},1\right\} \nonumber\\ 
{v_3}&= \left\{\frac{d^2-c\left(\lambda_{3}+b\right)}{-d(c+\lambda_{2})}-\frac{\lambda_{3}+b}{d},-\frac{d^2-c \left(\lambda_{3}+b\right)}{-\frac{1}{2} d \sqrt{a^2-2 a b+2 a c+b^2-2 b c+c^2+8 d^2}+\frac{a d}{2}-\frac{b d}{2}-\frac{3 c d}{2}},1\right\} \nonumber
\end{align}




==> leftovers/leftovers.tex <==
%%%%%Rayleigh
\subsection{Rayleigh approximation}

To obtain an explicit representation for the spectrum (\ref{spectrumdefinition}) and for the dispersion relation (\ref{dispersion}) from the general propagation condition (\ref{propa2}) is clearly an hopeless and somehow meaningless, as remarked into \cite{BANE17}, task.

We can obtain, however, an estimate for the spectrum of $M$ by the means of the \emph{generalized Rayleigh quotient} [CITARE]:
\begin{equation}\label{rayleigh}
F(w)=\frac{<Mw\,,w^{*}>}{<Jw\,,w^{*}>}\,;
\end{equation}
provided we define the \emph{numerical range} for $F(w)$ as the convex set $W(M\,,J)$ 
\begin{equation}
W(M\,,J)\equiv\Big\{F(w)=\frac{<Mw\,,w^{*}>}{<Jw\,,w^{*}>}\,|\,w\in C^{m}\,,\quad w\neq 0\Big\}\,,
\end{equation}
and since $M=M^{*}$, then $W(M\,,J)$ is the real interval bounded by $[\omega^{2}_{min}\,,\omega^{2}_{max}]$; accordingly:
\begin{equation}
\omega_{1}^{2}=\min_{w\in\caW_{1}/\{0\}} F(w)\,,\quad\caW_{1}\equiv\caV\oplus\Lin\,.
\end{equation}
We define a sequence of orthogonal vectors $w_{1}\,,w_{2}\,,\ldots w_{12}$:
\begin{equation}
w_{1}\in\caW_{1}\,,\quad w_{k}\in\caW_{k}\equiv\{w\in\caW_{k-1}\,|\,<w\,,w_{k-1}>=0\}\,,\quad k=2\,,\ldots\,,12\,,
\end{equation}
and then the ordered sequence of Rayleigh quotients $F(w_{k})$ is, element by element, an upper bound for the spectrum of $M$; moreover, the group and phase velocities can be trivially estimated from these frequency estimates by the definition (\ref{velocities}).

Now, when we write the elements of the complex vector $w$ in their most general form
\begin{equation}\label{wcomplex}
\ab=L_{m}(\ub+i\vb)\,,\quad\Cb=\Ub+i\Vb\,,
\end{equation}
we arrive from (\ref{rayleigh}) at
\begin{eqnarray}\label{raybigcomplex}
<Mw\,,w^{*}>&=&\xi^{2}\Big(\Ab\ub\cdot\ub+\Ab\vb\cdot\vb+\zeta_{1}^{2}(\Ael[\Ub]\cdot\Ub+\Ael[\Vb]\cdot\Vb)\nonumber\\
&+&2\zeta_{1}(\Pbm[\Ub]\cdot\ub+\Pbm[\Vb]\cdot\vb)\Big)\\
&+&2\xi L_{m}^{-1}(\Qbm[\Ub]\cdot\vb-\Qbm[\Vb]\cdot\ub)+L_{m}^{-2}(\bar{\Bel}[\Ub]\cdot\Ub+\bar{\Bel}[\Vb]\cdot\Vb)\,,\nonumber\\
<Jw\,,w^{*}>&=&\|\ub\|^{2}+\|\vb\|^{2}+\zeta_{2}^{2}(\hat{\Jel}[\Ub]\cdot\Ub+\hat{\Jel}[\Vb]\cdot\Vb)\,;\nonumber
\end{eqnarray}
we remark that, in order to give an estimate for the spectrum with (\ref{raybigcomplex}), we need to construct of a set of 12 orthogonal complex vectors into $\caW_{1}$ , a task which can be daunting. To this regard, an useful hint to simplify (\ref{raybigcomplex}) comes from the solutions we obtained in the long wavelength approximation, namely to assume real macroscopic displacements and purely immaginary microdistortions:
\begin{equation}\label{wcomplex2}
\ab=L_{m}\ub\,,\quad\Cb=i\Vb\,;
\end{equation}
hence (\ref{raybigcomplex}) reduces to
\begin{eqnarray}\label{raybigcomplex2}
F(w)=\frac{\xi^{2}\Big(\Ab\ub\cdot\ub+\zeta_{1}^{2}\Ael[\Vb]\cdot\Vb\Big)-2\xi L_{m}^{-1}\Qbm[\Vb]\cdot\ub+L_{m}^{-2}\bar{\Bel}[\Vb]\cdot\Vb}
{\|\ub\|^{2}+\zeta_{2}^{2}\hat{\Jel}[\Vb]\cdot\Vb}\,.
\end{eqnarray}

\begin{rmk}
In the long wavelength approximation the Rayleigh quotient reduces to
\begin{equation}\label{raymacro}
F(\ub)=\frac{\xi^{2}\hat{\Ab}\ub\cdot\ub}{\|\ub\|^{2}}\,,\quad\ub\in\caV\,,
\end{equation}
with $\ub$ a real valued vector, whereas in the microvibration case we have
\begin{equation}\label{rayleighboundmicro}
F(\Ub)=
\frac{\Bel[\Ub]\cdot\Ub}{\rho\Jel[\Ub]\cdot\Ub}\,,\quad\Ub\in\Lin\,,
\end{equation}
where $\Ub$ is a real valued tensor. By choosing in these cases a set of three real orthogonal vectors for (\ref{raymacro}) and a set of nine real orthogonal tensors for (\ref{rayleighboundmicro}) we can give a Rayleigh estimate for the associated spectrum. 
\end{rmk}


%%%%%%%%%%%%%%%






\begin{equation}\label{chara4}
\omega^{8}-B(\xi)\omega^{6}+C(\xi)\omega^{4}+D(\xi)\omega^{2}+E(\xi)=0\,,
\end{equation}
whose coefficients depend on the wavenumber $\xi$ in the following way:
\begin{align}
B(\xi)&=\xi^{2}b_{1}+b\,,\nonumber\\
C(\xi)&=\xi^{4}c_{2}+\xi^{2}c_{1}+c\,,\nonumber\\
D(\xi)&=\xi^{6}d_{3}+\xi^{4}d_{2}+\xi^{2}d_{1}+d\,,\nonumber\\
E(\xi)&=\xi^{8}e_{4}+\xi^{6}e_{3}+\xi^{4}e_{2}+\xi^{2}e_{1}\,,\nonumber
\end{align}
where 
\begin{align}
b_{1}&=A_{33}+\hat{\Ael}_{33}+2\hat{\Ael}_{11}\,,\nonumber\\
c_{1}&=A_{33}(\hat{\Bel}_{33}-2\hat{\Bel}_{11})+\hat{\Ael}_{11}\hat{\Bel}_{33}+\hat{\Ael}_{33}\hat{\Bel}_{11}-2\hat{\Ael}_{13}\hat{\Bel}_{13}+2\hat{\Ael}_{11}\hat{\Bel}_{11}-2\hat{\Ael}_{12}\hat{\Bel}_{12}\nonumber\\
&+2(\hat{\Qbm}_{311}^{2}-\hat{\Qbm}_{333}^{2})\,,\nonumber\\
c_{2}&=A_{33}(\hat{\Ael}_{33}-2\hat{\Ael}_{11})+\hat{\Ael}_{11}\hat{\Ael}_{33}-\hat{\Ael}_{13}^{2}+\hat{\Ael}_{11}^{2}-\hat{\Ael}_{12}^{2}+2(\hat{\Pbm}_{311}^{2}-\hat{\Pbm}_{333}^{2})\,,\nonumber\\
d_{1}&=\,,\nonumber\\
d_{2}&=\,,\\
d_{3}&=\,,\nonumber\\
e_{1}&=\,,\nonumber\\
e_{2}&=\,,\nonumber\\
e_{3}&=\,,\nonumber\\
e_{4}&=\,,\nonumber
\end{align}
and with  $b$, $c$ and $d$  given by the relations (\ref{coefficubic}) and:
\begin{align}
&\hat{\Ael}_{11}=\frac{\Ael_{11}L_{c}^{2}}{J_{11}}\,,\quad\hat{\Ael}_{33}=\frac{\Ael_{33}L_{c}^{2}}{J_{33}}\,,\quad\hat{\Ael}_{12}=\frac{\Ael_{12}L_{c}^{2}}{\sqrt{J_{11}J_{33}}}\,,\quad\hat{\Ael}_{13}=\frac{\Ael_{13}L_{c}^{2}}{\sqrt{J_{11}J_{33}}}\,,\nonumber\\
&\hat{\Pbm}_{311}=\frac{\Pbm_{311}L_{c}^{2}}{L_{m}\sqrt{J_{11}}}\,,\quad\hat{\Pbm}_{333}=\frac{\Pbm_{333}L_{c}^{2}}{L_{m}\sqrt{J_{33}}}\,,\quad\hat{\Qbm}_{311}=\frac{\Qbm_{311}}{\sqrt{J_{11}}}\,,\quad\hat{\Qbm}_{333}=\frac{\Qbm_{333}}{\sqrt{J_{33}}}\,
\end{align}

[VEDERE LA DIPENDENZA DA LM e dai vari parametri]

The explicit solution can be then obtained by one of the explicit formulae based on the Cardano's formulae, for instance with:
\begin{align}\label{cardano4}
\omega^{2}_{1,2}(\xi)=\frac{B(\xi)}{4}-Q\pm\sqrt{\frac{3}{4}B^{2}(\xi)-2C(\xi)-4Q^{2}-\frac{S}{Q}}\,,\\
\omega^{2}_{3,4}(\xi)=\frac{B(\xi)}{4}+Q\pm\sqrt{\frac{3}{4}B^{2}(\xi)-2C(\xi)-4Q^{2}+\frac{S}{Q}}\,.\nonumber
\end{align}

To investigate about the behaviour of (\ref{cardano4}) for $\xi\rightarrow 0$ we notice that, since $B(0)=b$, $C(0)=c$, $D(0)=d$ and $E(0)=0$, then the characteristic equation (\ref{chara4}) reduces to
\begin{equation}
\omega^{2}(\omega^{6}-b\omega^{4}+c\omega^{2}+d)=0\,,
\end{equation}
which admits the three solutions (\ref{cardano3}) (the cut-off for the three optic frequencies into (\ref{cardano4})) and a frequency $\omega^{2}=0$ which corresponds, into the limit, to $\ab=\bzero$. Therefore into the subspace $\caN_{1}$ we have three optic and one acoustic frequencies, this one corresponding to a longitudinal macroscopic wave. The four associated eigenvectors, which have the form [VEDERE SE E' VERO]
\begin{align}
w_{k}(\xi)\equiv\{a_{k}(\xi)\eb_{3}\,; \Cb_{k}(\xi)=C_{1k}(\xi)\Wb_{1}+C_{2k}(\xi)\Wb_{2}+C_{3k}(\xi)\Wb_{3}\}\,,
\end{align}
for $k=1,2,3,4$, reduces into the limit for $\xi\rightarrow 0$ to the three eigenvectors (\ref{treeigenHS}) with $a_{k}=0$ and $C_{j4}=0$, $j=1,2,3$.


%%%%%%%%%%%%%%%%%%%

If we furthermore define
\begin{equation}
\bar{\Jb}=\Gb\Jb\Gb^{T}\,,
\end{equation}
which yields
\begin{equation}
(\bar{\Jb})\dot{}=\Wb\bar{\Jb}+\bar{\Jb}\Wb\,,
\end{equation}
where a new kinematical quantity, the \emph{whorl} \cite{CPW82}, is introduced:
\begin{equation}
\Wb=\dot{\Gb}\Gb^{-1}\,,
\end{equation}
then we can rewrite (\ref{system1})$_{2}$ as:
\begin{equation}\label{system2}
\dive\Hbm+\Sbb+\bar{\Bb}=\rho\bar{\Jb}(\dot{\Wb}+\Wb^{2})^{T}\,.
\end{equation} 

whereas the phase velocities (\ref{velocities})$_{2}$ can determined by using a result given in \cite{LA64}:
\begin{equation}
v_{k}^{g}(\xi_{o})=\frac{1}{2\omega_{k}(\xi_{o})}<\frac{\dif M}{\dif\xi}\Big|_{\xi=\xi_{o}}w_{k}(\xi_{o})\,,w^{*}_{k}(\xi_{o})>\,.
\end{equation}

\begin{rmk}[PWO]

The Lead Tungstenate PbWO$_{4}$ (PWO) is a tetragonal crystal of the class $4/m$ whose density is $\rho=8.28$ g/cm$^{3}$ and whose elasticities are (in GPa) \cite{KO96}: 
\begin{eqnarray*}
&\Cel_{1111}=107.7\,,\quad\Cel_{1122}=70.1\,,\quad\Cel_{3333}=93.7\,,\quad\Cel_{1133}=49.1\,,\\
&\Cel_{2323}=25\,,\quad\Cel_{1212}=40.6\,,\quad\Cel_{1112}=-12\,;\nonumber
\end{eqnarray*}
with these data the propagation velocities for an acoustic wave propagating along the $c-$axis, by (\ref{wavecaxis}) are (in m/sec):
\begin{equation*}
c_{L}=3363>c_{T}=1838\,,
\end{equation*}
As far as the propagation in directions which are orthogonal to the $c-$axis, for an angle $\theta=0.078$ rad. we have a longitudinal and two transverse waves with velocities and amplitudes:
\begin{equation*}
(c_{1,T}=2250\,,\ab_{1}=\eb_{3}\times\mb)\,,\quad(c_{2,T}=3363\,,\ab_{2}=\eb_{3})\,,\quad(c_{3,L}=3583\,,\ab_{3}=\mb)\,.
\end{equation*}
\end{rmk}

%%%%%%%%%%%%%%%%%%%%

\begin{equation}\label{QBM1}
[\Qbm(\eb_{3})]=
\left[
\begin{array}{ccccccccc}
0 &  0  & 0  & \Qbm_{123} & \Qbm_{131} & 0 & \Qbm_{132} & \Qbm_{113} & 0\\
 0 &  0 & 0 & \Qbm_{113} & -\Qbm_{132}& 0 & -\Qbm_{131}& -\Qbm_{123}& 0\\
\Qbm_{311} &  \Qbm_{311}  &  \Qbm_{333}  & 0& 0& \Qbm_{312}& 0&0& -\Qbm_{312}
\end{array}
\right]
\end{equation}
where the independent components are given by:
\begin{eqnarray}\label{QBM2}
\Qbm_{123}&=&\rho^{-1}\Bel_{1233}\,,\nonumber\\
\Qbm_{131}&=&\rho^{-1}(\Del_{2323}+\Bel_{2323})\,,\nonumber\\
\Qbm_{132}&=&\rho^{-1}\Del_{3123}\,,\nonumber\\
\Qbm_{113}&=&\rho^{-1}(\Del_{1133}+\Bel_{1133})\,,\\
\Qbm_{311}&=&\rho^{-1}(\Del_{2323}+\Bel_{2332})\,,\nonumber\\
\Qbm_{333}&=&\rho^{-1}(\Del_{3333}+\Bel_{3333})\,,\nonumber\\
\Qbm_{312}&=&\rho^{-1}(\Del_{3123}+\Bel_{3123})\,;\nonumber
\end{eqnarray}

\begin{equation}\label{QBM3}
[\Qbm(\theta)]=
\left[
\begin{array}{ccccccccc}
\Qbm_{111} &  \Qbm_{122}  & \Qbm_{333}  & 0 & 0 & \Qbm_{112} & 0 & 0 & \Qbm_{121}\\
\Qbm_{211} &  \Qbm_{222} & \Qbm_{233} & 0& 0 & \Qbm_{212} & 0 & 0 & \Qbm_{221}\\
0 &  0  &  0  & \Qbm_{323}& \Qbm_{331}& 0 & \Qbm_{332}&\Qbm_{313}& 0
\end{array}
\right]
\end{equation}
with
For all the classes $4$, $\bar{4}$ and $4/m$ the non-null components of $\Qbm$ are

\begin{eqnarray}
\Qbm_{111}&=&(\Del_{1111}+\Bel_{1111})\cos\theta+(\Del_{1112}+\Bel_{1112})\sin\theta\,,\nonumber\\
\Qbm_{122}&=&(\Del_{1212}+\Bel_{1221})\cos\theta+(-\Del_{2111}+\Bel_{1222})\sin\theta\,,\nonumber\\
\Qbm_{133}&=&(\Del_{3131}+\Bel_{2332})\cos\theta-(\Del_{2331}+\Bel_{2331})\sin\theta\,,\nonumber\\
\Qbm_{123}&=&0\,,\nonumber\\
\Qbm_{131}&=&0\,,\nonumber\\
\Qbm_{112}&=&-(\Del_{2212}+\Bel_{2212})\cos\theta+(\Del_{1122}+\Bel_{1122})\sin\theta\,,\nonumber\\
\Qbm_{132}&=&0\,,\nonumber\\
\Qbm_{113}&=&0\,,\nonumber\\
\Qbm_{121}&=&(\Del_{1211}+\Bel_{1211})\cos\theta+(\Del_{1212}+\Bel_{1212})\sin\theta\,,\nonumber\\
\Qbm_{211}&=&(\Del_{1211}-\Bel_{2212})\cos\theta+(\Del_{1212}+\Bel_{2112})\sin\theta\,,\nonumber\\
\Qbm_{222}&=&-(\Del_{1112}+\Bel_{1112})\cos\theta+(\Del_{1111}+\Bel_{1111})\sin\theta\,,\nonumber\\
\Qbm_{233}&=&(\Del_{2331}+\Bel_{2331})\cos\theta+(\Del_{3131}+\Bel_{2332})\sin\theta\,,\nonumber\\
\Qbm_{223}&=&0\,,\nonumber\\
\Qbm_{231}&=&0\,,\\
\Qbm_{212}&=&(\Del_{1212}+\Bel_{2121})\cos\theta+(-\Del_{1211}+\Bel_{2122})\sin\theta\,,\nonumber\\
\Qbm_{232}&=&0\,,\nonumber\\
\Qbm_{213}&=&0\,,\nonumber\\
\Qbm_{221}&=&(\Del_{1122}+\Bel_{2211})\cos\theta+(\Del_{2212}+\Bel_{2212})\sin\theta\,,\nonumber\\
\Qbm_{311}&=&0\,,\nonumber\\
\Qbm_{322}&=&0\,,\nonumber\\
\Qbm_{333}&=&0\,,\nonumber\\
\Qbm_{323}&=&\Del_{2331}\cos\theta+(\Del_{3131}+\Bel_{2323})\sin\theta\,,\nonumber\\
\Qbm_{331}&=&(\Del_{3311}+\Bel_{3311})\cos\theta+(\Del_{3312}+\Bel_{3312})\sin\theta\,,\nonumber\\
\Qbm_{312}&=&0\,,\nonumber\\
\Qbm_{332}&=&-(\Del_{3312}+\Bel_{3312})\cos\theta+(\Del_{3311}+\Bel_{3311})\sin\theta\,,\nonumber\\
\Qbm_{313}&=&(\Del_{3131}+\Bel_{3131})\cos\theta-\Del_{2331}\sin\theta\,,\nonumber\\
\Qbm_{321}&=&0\,;\nonumber
\end{eqnarray}

begin{equation}
%M\equiv
\left[
\begin{array}{cccccccccccc}
B_{11}  & B_{12}  & 0  &0 &  0  & 0  & \Rbm_{123} & \Rbm_{131} & 0 & \Rbm_{132} & \Rbm_{113} & 0\\
B_{12} & B_{11}  & 0  & 0 &  0 & 0 & \Rbm_{113}& -\Rbm_{132}& 0 & -\Rbm_{131}& -\Rbm_{123}& 0\\
0 & 0 &  B_{33} &  \Rbm_{311} &  \Rbm_{311}  &  \Rbm_{333}  & 0& 0& \Rbm_{312}& 0&0& -\Rbm_{312}\\
0& 0& \bar{\Rbm}_{311} & \Sel_{11} & \Sel_{12} & \Sel_{13} & 0 & 0 & \Sel_{16} & 0 & 0 & -\Sel_{26}\\
0& 0& \bar{\Rbm}_{311}& \Sel_{12}& \Sel_{11} & \Sel_{13} & 0 & 0 & \Sel_{26} & 0 & 0 & -\Sel_{16}\\
0& 0& \bar{\Rbm}_{333} &\Sel_{13} & \Sel_{13}& \Sel_{33} & 0 & 0 & \Sel_{36} & 0 & 0 & -\Sel_{36}\\
\bar{\Rbm}_{123}& \bar{\Rbm}_{113}& 0 & 0 & 0 &  0 & \Sel_{44} & \Sel_{45} & 0 & \Sel_{47} & \xi^{2}\Ael_{48} & 0\\
\bar{\Rbm}_{131}& -\bar{\Rbm}_{132}& 0 & 0 & 0 & 0&  \Sel_{45} & \Sel_{55} & 0 & \xi^{2}\Ael_{57} & \Sel_{47} & 0\\
0& 0& \bar{\Rbm}_{312}& \Sel_{16}  & \Sel_{26} & \Sel_{36}& 0& 0& \Sel_{66} & 0 & 0 & \Sel_{69}\\
\bar{\Rbm}_{132}& -\bar{\Rbm}_{131}& 0& 0& 0 & 0 & \Sel_{47} &  \xi^{2}\Ael_{57} &  0 & \Sel_{55} & -\Sel_{45} & 0\\
\bar{\Rbm}_{113}& -\bar{\Rbm}_{123}& 0 & 0 & 0 & 0 & \xi^{2}\Ael_{48}& \Sel_{47} & 0 &  -\Sel_{45} & \Sel_{44} & 0\\
0& 0&-\bar{\Rbm}_{312} & -\Sel_{26} & -\Sel_{16}& -\Sel_{36} & 0 & 0 & \Sel_{69} &  0& 0& \Sel_{66}
\end{array}
\right]\,,
\end{equation}

\begin{equation}
%M\equiv
\left[
\begin{array}{cccccccccccc}
B_{1}  & B_{6}  & 0  &0 &  0  & 0  & \Rbm_{14} & \Rbm_{15} & 0 & \Rbm_{17} & \Rbm_{18} & 0\\
B_{6} & B_{1}  & 0  & 0 &  0 & 0 & \Rbm_{18}& -\Rbm_{17}& 0 & -\Rbm_{15}& -\Rbm_{14}& 0\\
0 & 0 &  B_{3} &  \Rbm_{31} &  \Rbm_{31}  &  \Rbm_{33}  & 0& 0& \Rbm_{36}& 0&0& -\Rbm_{36}\\
0& 0& \bar{\Rbm}_{31} & \Sel_{11} & \Sel_{12} & \Sel_{13} & 0 & 0 & \Sel_{16} & 0 & 0 & -\Sel_{26}\\
0& 0& \bar{\Rbm}_{31}& \Sel_{12}& \Sel_{11} & \Sel_{13} & 0 & 0 & \Sel_{26} & 0 & 0 & -\Sel_{16}\\
0& 0& \bar{\Rbm}_{33} &\Sel_{13} & \Sel_{13}& \Sel_{33} & 0 & 0 & \Sel_{36} & 0 & 0 & -\Sel_{36}\\
\bar{\Rbm}_{14}& \bar{\Rbm}_{18}& 0 & 0 & 0 &  0 & \Sel_{44} & \Sel_{45} & 0 & \Sel_{47} & \xi^{2}\Ael_{48} & 0\\
\bar{\Rbm}_{15}& -\bar{\Rbm}_{17}& 0 & 0 & 0 & 0&  \Sel_{45} & \Sel_{55} & 0 & \xi^{2}\Ael_{57} & \Sel_{47} & 0\\
0& 0& \bar{\Rbm}_{36}& \Sel_{16}  & \Sel_{26} & \Sel_{36}& 0& 0& \Sel_{66} & 0 & 0 & \Sel_{69}\\
\bar{\Rbm}_{17}& -\bar{\Rbm}_{15}& 0& 0& 0 & 0 & \Sel_{47} &  \xi^{2}\Ael_{57} &  0 & \Sel_{55} & -\Sel_{45} & 0\\
\bar{\Rbm}_{18}& -\bar{\Rbm}_{14}& 0 & 0 & 0 & 0 & \xi^{2}\Ael_{48}& \Sel_{47} & 0 &  -\Sel_{45} & \Sel_{44} & 0\\
0& 0&-\bar{\Rbm}_{36} & -\Sel_{26} & -\Sel_{16}& -\Sel_{36} & 0 & 0 & \Sel_{69} &  0& 0& \Sel_{66}
\end{array}
\right]\,,
\end{equation}
where we denote $B_{ij}=\xi^{2}A_{ij}$, $\Rbm_{ijk}=\xi^{2}\Pbm_{ijk}+i\xi\Qbm_{ijk}$ and $\Sel_{AB}=\xi^{2}\Ael_{AB}+\Bel_{AB}$; here the components $A_{ij}$ are given by (\ref{acoustic1LS}) evaluated for $m_{1}=m_{2}=0$ and $m_{3}=1$, whereas the non-null components of $\Pbm$ and $\Qbm$ are given by () and () and those of $\Ael_{AB}$ by ().

%%%%%%%%%%%%%%%%%%
\begin{equation}
\renewcommand{\arraystretch}{1.5} % give some more room
M\equiv
\left[\begin{array}{@{}ccc|ccccccccc@{}}
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\ \hline
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot 
\end{array}\right]\,,
\end{equation}

High-symmetries
\begin{equation}
\renewcommand{\arraystretch}{1.5} % give some more room
M\equiv
\left[\begin{array}{@{}ccc|ccccccccc@{}}
\bullet&\bullet&\cdot&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet&\cdot \\
\bullet&\bullet&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet&\cdot&\cdot \\
\cdot&\cdot&\bullet&\bullet&\bullet&\bullet&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\ \hline
\cdot&\cdot&\bullet&\bullet&\bullet&\bullet&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\bullet&\bullet&\bullet&\bullet&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\cdot&\bullet&\bullet&\bullet&\bullet&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot \\
\cdot&\bullet&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet&\cdot&\cdot \\
\bullet&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet \\
\cdot&\bullet&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet&\cdot&\cdot \\
\bullet&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet&\cdot \\
\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\cdot&\bullet&\cdot&\cdot&\bullet
\end{array}\right]\,,
\end{equation}

%%%%%%%%


\begin{center}
\begin{tikzpicture}[>=triangle 60]
  \matrix[matrix of math nodes,column sep={90pt,between origins},row
    sep={50pt,between origins},nodes={asymmetrical rectangle}] (s)
  {
    & &|[name=kb]| \caN_{1} &|[name=kc]| \caZ_{1}+AL \\
    
    |[name=U]| AL+\caU_{1} &|[name=A]| \caM_{1} &|[name=B]| \caN_{2}&|[name=C]| \caZ_{2} \\
    
    |[name=02]| AT+\caU_{2} &|[name=A']| \caM_{2} &|[name=B']| \caN_{3} &|[name=C']| \caZ_{3}+AT \\
    
    &|[name=ca]| f &|[name=cb]| g &|[name=cc]|  h \\
  };
\draw[->] 
(B) edge node[auto] {\($\xi\rightarrow 0$\)} (C)
(A) edge node[auto] {\($\xi\rightarrow 0$\)} (U)
(AÕ) edge node[auto] {\($\xi\rightarrow 0$\)} (02)
(BÕ) edge node[auto] {\($\xi\rightarrow 0$\)} (C')
(kb) edge node[auto] {\($\xi\rightarrow 0$\)} (kc)
;
\draw[<->, gray]  
(A) edge (kb)  
(A) edge (B)
(AÕ) edge (B')         
;
\end{tikzpicture}

\caption{prova}
\end{center}





